Characterizations of compactness and weighted eigenvalue problem associated with fractional Hardy-type inequalities

In this article, we consider the following fractional {Hardy-type} inequality: \begin{align} \label{Fractional Hardy_abst} \int_{\mathbb{R}^N} |w(x)||u(x)|^p \mathrm{d}x \leq C \int_{\mathbb{R}^N \times \mathbb{R}^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} \mathrm{d}x\mathrm{d}y:= \|u\|_{s,p}^p\,, \ \forall u \in \mathcal{D}^{s,p}(\mathbb{R}^N), \end{align} where $0<s<1<p<\frac{N}{s}$, and $\mathcal{D}^{s,p}(\mathbb{R}^N)$ is the completion of $C_c^1(\mathbb{R}^N)$ with respect to the {norm} $\|\cdot\|_{s,p}$. We denote the space of admissible {weight function} $w$ in \eqref{Fractional Hardy_abst} by $\mathcal{H}_{s,p}(\mathbb{R}^N)$. Maz'ya-type characterization helps us to define a Banach function norm on $\mathcal{H}_{s,p}(\mathbb{R}^N)$. Using the Banach function space structure and the concentration compactness type arguments, we provide several characterizations for the compactness of the map ${W}(u)= \int_{{\mathbb{R}^N}} |w| |u|^p \mathrm{d}x$ on $\mathcal{D}^{s,p}(\mathbb{R}^N)$. In particular, we prove that ${W}$ is compact on $\mathcal{D}^{s,p}(\mathbb{R}^N)$ if and only if $w \in \mathcal{H}_{s,p,0}(\mathbb{R}^N):=\overline{C_c(\mathbb{R}^N)} \ \mbox{in} \ \mathcal{H}_{s,p}(\mathbb{R}^N)$. Further, we study the following {weighted} eigenvalue problem: \begin{equation*} (-\Delta_{p})^{s}u = \lambda w(x) |u|^{p-2}u ~~\text{in}~\mathbb{R}^{N}, \end{equation*} where $(-\Delta_{p})^{s}$ is the fractional $p$-Laplace operator and $w = w_{1} - w_{2}~\text{with}~ w_{1},w_{2} \geq 0,$ is such that $ w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^N)$ and $w_{2} \in L^{1}_{loc}(\mathbb{R}^N)$.

==> Results.tex <==
\section{Compactness of the energy functional} \label{Compactness}
 {In this section, we prove our main result Theorem \ref{allinone1}. We divide the section into several subsections and develop the required tools for proving Theorem \ref{allinone1}. Indeed, each subsection contains certain results that are independently significant in their
own right.}
%\subsection{Tools needed}
%Fractional order capacity, Mazya's capacity condition, fractional concentration compactness.
%\subsection{Tools available}
%Fractional order capacity \cite{Xiao}, Mazya's capacity condition \cite{Dyda}.
%\vspace{1cm} 
% Let $0<s<1$ and $1<p<\frac{N}{s}$. In this paper, we are interested in the following fractional Hardy inequality:
% \begin{align} \label{FHardy}
%   \int_{\R^N} w(x)|u(x)|^p  \dx \leq C  \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}}\dxy:= \norm{u}_{s,p}^p\,, \ \forall u \in \mathcal{D}^{s,p}_0(\R^N) 
% \end{align}
% where $w \in L^1_{loc}(\R^N)$ and $ \mathcal{D}^{s,p}_0(\R^N)$ is the completion of $C_c^{1}(\R^N)$ with respect to $\norm{u}_{s,p}.$ 


% {\color{red} \begin{definition}
% Let $\Om$ be an open set in $\R^N.$ For any $K \subset \subset \Om$, we define
% \begin{align*}
%     {\rm{Cap}}_{s,p}(K,\Om)=\inf \big\{\norm{u}_{s,p,\Om}^p: u \in C_c^1(\Om), 0\leq u \leq 1, u = 1 \ \mbox{on} \ K \big\}\,,
% \end{align*}
% where $\displaystyle \|u\|_{s,p,\Om}^p=\int_{\Om \times \Om} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}}$.

% \noi For $\Om=\R^N$, we write ${\rm{Cap}}_{s,p}(K,\R^N)$ as ${\rm{Cap}}_{s,p}(K)$.
% \end{definition}
% \noi Let $w$ satisfies \eqref{FHardy}. Now, if $u \in C_c^1(\R^N), 0\leq u \leq 1, u = 1 \ \mbox{on} \ K,$ then 
% $$\int_{K} |w(x)| \ dx \leq \int_{\R^N} |w(x)| |u(x)|^p \ dx  \leq C \norm{u}_{s,p}^p$$
% This implies $\int_{K} |w(x)| \ dx   \leq C \mathrm{Cap}_{s,p}(K,\R^N).$ Therefore, $w$ necessarily satisfies
% \begin{align*}
%     \sup_{K \subset \subset \R^N} \frac{\int_{K} |w(x)| \ dx}{\mbox{Cap}_{s,p}(K,\R^N)} < \infty.
% \end{align*}
% In fact, this condition is also sufficient for $w$ to satisfies \eqref{FHardy}.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Mazya's capacity condition } Let $s \in (0,1)$, $p \in (1,\infty)$ and $sp<N$. Then, by \cite[Proposition 3.1]{Dyda} $w$ satisfies \eqref{FHardy} iff 
% \begin{align}
%     \sup_{K \subset \subset \R^N} \frac{\int_{K} |w(x)| \ dx}{\mbox{Cap}_{s,p}(K,\R^N)} < \infty.
% \end{align}
%   Motivated by this, for $w \in L^1_{loc}(\R^N)$, we define
% \begin{align}
%  \norm{w}_{\mathcal{H}_{s,p}} =  \sup_{K \subset \subset \R^N} \frac{\int_{K} |w(x)| \ dx}{\mbox{Cap}_{s,p}(K,\R^N)} < \infty.
% \end{align}
% Indeed, $ \norm{.}_{\mathcal{H}_{s,p}}$ is a Banach function space norm on
% $$\mathcal{H}_{s,p}(\R^N):=\big\{w \in L^1_{loc}(\R^N): \norm{w}_{\mathcal{H}_{s,p}} < \infty \big\} \,.$$
% For any $w \in \mathcal{H}_{s,p}(\R^N)$, we consider the following concentration function of $w$:
%  \begin{eqnarray*}
%   \C_w(x)= \lim_{r \ra 0}  \norm{w \chi_{ B_r(x)}}_{\mathcal{H}_{s,p}} , \qquad 
%   \C_w({\infty}) =\lim_{R \ra \infty} \norm{w \chi_{ {B}_R(0)^c}}_{\mathcal{H}_{s,p}}. 
%  \end{eqnarray*}
% % \begin{align*}
% %     \C_w(x)= \lim_{r \ra 0} \norm{w \chi_{B_r(x)}}_{\mathcal{H}}; \, x \in \overline{\R^N}\,, \quad \quad
% We define the singular set of $w$ as $\sum_w=\{x \in \R^N: \C_w(x) > 0\}$. }

% Next, we obtain a result that 
\subsection{\tb{Characterization} of the Hardy potentials}
% Let $\phi$ be a non-decreasing function such that $\phi(t)>0$ for $t>0$ and $\phi$ is continuous from the right for $t \geq 0$. Further, $\phi$ satisfies $\phi(0)=0$, $\phi(t) \to \infty$ as $t \to \infty$. Let the function \tb{$M(r)$} admit the following representation:
% \begin{align*}
%   \tb{  M(r)=\int_{0}^{|r|} \phi(t)\,\mathrm{d} t.}
% \end{align*}
% The functions admitting the above representation are known as the Young function. In particular, $M$ is a Young function. Further, we define the right inverse of $\phi(t)$ as
% \begin{align*}
%     \psi(s)= \sup\{t: \phi(t) \leq s\}.
% \end{align*} 
% The function
% \begin{align*}
%  \tb{  P(r)=\int_0^{|r|} \psi(s)\, \mathrm{d}s }
% \end{align*}
% is known as the complementary function to \tb{$M(r)$}. We refer to the book \cite{Mazya} for more details on this topic. Further, we define a space associated with a Young function $M$. Let $\mathcal{L}_M(\Omega,\mu)$ be the space of all $\mu$-measurable functions such that
% \begin{align*}
%     \norm{u}_{\mathcal{L}_M(\Omega,\mu)} = \sup \left\{\left|\int_{\Omega}uv\,\mathrm{d} \mu\right|: \int_{\Omega}P(v)\,\mathrm{d} \mu \leq  1 \right\}< \infty.
% \end{align*}
 % {The following result} is a by-product of fractional Maz’ya-type characterization of Hardy potentials. 
 Let us first recall the Maz’ya-type characterization of fractional-Hardy-weights. For a proof we refer to \cite[Proposition 5]{Dyda}.
\begin{theorem} \label{H1}
Let  {$0<s<1<p<\frac{N}{s}$ and} $w \in L^{1}_{loc}(\R^N)$. If $ w \in \mathcal{H}_{s,p}(\mathbb{R}^{N})$, then $$\int_{\R^N} w |u|^{p} \dx \leq C_{H} \|w\|_{\mathcal{H}_{s,p}} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}} \dxy,~\forall ~ u \in \mathcal{D}_{}^{s,p}(\mathbb{R}^{N}).$$
\end{theorem}
% \begin{proof}
% Suppose $ U_{t} = \{ x \in \R^N : |u(x)| \geq t \} $. 
% Now by \cite[Sect. 2.3.2]{Mazya} we have 
% \begin{eqnarray*}
%  \|~|u|^{p}\|_{\mathcal{L}_{M}(\R^N,\mu)} & = &\mbox{sup} \bigg\{~\bigg|\int_{\R^N} w |u|^{p} \dm \bigg| : \int_{\R^N} P(w) \dm \leq 1 \bigg\}\\
%   &=& \mbox{sup} \bigg\{\int_{0}^{\infty} \int_{U_{t}} w ~\dm ~\mathrm{d}({t}^{p}) : \int_{\R^N} P(w) \dm \leq 1 \bigg\}\\
%    & \leq& \int_{0}^{\infty} \mbox{sup} \bigg\{ \int_{\R^N} \displaystyle\chi_{U_{t}} w ~\dm  : \int_{\R^N} P(w) \dm \leq 1 \bigg\} ~\mathrm{d}({t}^{p})~ \\
%    & = &  \int_{0}^{\infty} \|\chi_{U_{t}}\|_{\mathcal{L}_{M}(\R^N,\mu)}~\mathrm{d}({t}^{p})  \\
%     &\leq& \|w\|_{\mathcal{H}_{s,p}(\R^N)} \int_{0}^{\infty} {\rm Cap_{s,p}}(U_{t})~\mathrm{d}({t}^{p})\\
%     &\leq& C_{H} \|w\|_{\mathcal{H}_{s,p}(\R^N)} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}} \dxy.
% \end{eqnarray*}
%  Hence, we get the desired result, where the last inequality is followed by 
%  \cite[Theorem 1$'$]{Wu}.
% \end{proof}
The next proposition gives an interesting property of the $(s,p)$-capacity. 
\begin{proposition} \label{propofcap}
   {Let $0<s<1<p<\frac{N}{s}$.} There exists $C_1, C_2 >0$ such that for a \tb{compact set} $F  \subset \R^N,$ 
   \begin{enumerate}[(i)]
    \item $ {\rm{Cap}}_{s,p}(F \cap \tb{\overline{B_r(x)}}, B_{2r}(x)) \leq C_1 {\rm{Cap}}_{s,p}(F \cap \tb{\overline{B_r(x)}}, \R^N),\ \forall r>0.$
    \item ${\rm{Cap}}_{s,p}(F \cap B_{2R}^c, \overline{B_R}^c) \leq C_2 {\rm{Cap}}_{s,p}(F \cap B_{2R}^c, \R^N), \ \forall R>0.$
   \end{enumerate}
\end{proposition}
\begin{proof}
$(i)$ Fix $x_0 \in \R^N$ and choose $\epsilon >0$ arbitrarily. Then, there exists $u \in C_c^1(\R^N)$ with $u \geq 1 $ a.e. in $F \cap \tb{\overline{B_r(x_0)}}$ such that 
$$\int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} \dxy < \mbox{Cap}_{s,p}(F \cap \tb{\overline{B_r(x_0)}}, \R^N) + \epsilon \,.$$
Take $\phi \in C_c^{\infty}(\R^N)$ such that $0 \leq \phi \leq 1$, $\phi =1$ on $\overline{B_1(0)}$ and vanishes outside $B_2(0)$. Consider $v_r=u \phi_{x_0,r}$, where $\phi_{x_0,r}(y)=\phi(\frac{y-x_0}{r})$. Note that, $v_r \geq 1$ on $F \cap \tb{\overline{B_r(x_0)}}$. Now
\begin{align*}
 & \, \int_{\R^N \times \R^N} \frac{|v_{r}(x)-v_{r}(y)|^p}{|x-y|^{N+sp}} \dxy \\
 & \leq \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}}\dxy + \int_{\R^N \times \R^N} |u(y)|^p \frac{|\phi_{x_0,r}(x)-\phi_{x_0,r}(y)|^p}{|x-y|^{N+sp}} \dxy\\
 & := I_1 + I_2 \,.
\end{align*}
We estimate $I_2$ as follows.
\begin{eqnarray*}
    I_2  & = & \int_{\R^N} |u(y)|^p \int_{\R^N} \frac{|\phi_{x_0,r}(x)-\phi_{x_0,r}(y)|^p}{|x-y|^{N+sp}} \ \dx  \dy \\
 & = & \int_{\R^N} |u(y)|^p \int_{\R^N} \frac{|\phi_{x_0,r}(y+z)-\phi_{x_0,r}(y)|^p}{|z|^{N+sp}} \ \mathrm{d}z \dy  \\
  & \leq & \int_{\R^N} |u(y)|^p |D^s \phi_{x_0,r}(y)|^p   \dy \\
  & = & \frac{1}{r^{sp}} \int_{\R^N} |u(y)|^p |D^s \phi(\frac{y-x_0}{r})|^p  \dy \ \ \mbox{  \cite[Lemma \ 2.1]{Bonder}}  \\
  & \leq & \|D^s \phi\|_{\infty}^p \left( \int_{\R^N} |u(y)|^{p_s^*}  \dy \right)^{\frac{N-sp}{N}} \left( \int_{\R^N} \left|\frac{D^s \phi(y)}{\|D^s \phi\|_{\infty}} \right|^{\frac{N}{s}}   \dy  \right)^{\frac{sp}{N}} \\
  & \leq & \|D^s \phi\|_{\infty}^p \left( \int_{\R^N} |u(y)|^{p_s^*} \dy \right)^{\frac{N-sp}{N}} \left( \int_{\R^N} \left|\frac{D^s \phi(y)}{\|D^s \phi\|_{\infty}} \right|^{p}   \dy  \right)^{\frac{sp}{N}} \\
  & \leq & C  \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}}  \dx  \dy
  \ = \ C I_1 \ \ \ \mbox{[by Remark \ref{infestimate}]}\,.
\end{eqnarray*}
  Thus, we obtain
  \begin{align*}
      \mbox{Cap}_{s,p}(F \cap B_r(x_0),  B_{2r}(x_0)) & \leq \int_{\R^N \times \R^N} \frac{|v_{r}(x)-v_{r}(y)|^p}{|x-y|^{N+sp}}\dxy 
       \leq (1+C) I_1 \\ & <C_{1}\mbox{Cap}_{s,p}(F \cap B_r(x_0), \R^N) +C_{1} \epsilon \,,
  \end{align*}
 where $C_{1} = 1+C.$ By taking $\epsilon \ra 0$, we prove $(i).$
  
  $(ii)$ Choose $\epsilon >0$ arbitrarily. Then there exists $u \in C_c^1(\R^N)$ with $u \geq 1 $ a.e. in $F \cap B_{2R}(0)^c$ such that 
$$\int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} \dxy< \mbox{Cap}_{s,p}(F \cap B_{2R}(0)^c, \R^N) + \epsilon \,.$$
Take $\phi \in C_b^{\infty}(\R^N)$ such that $0 \leq \phi \leq 1$, $\phi =0$ on $B_1(0)$ and $\phi =1$ on $B_2(0)^c$. Consider $v_{R}=u \phi_{R}$, where $\phi_{R}(x)=\phi(\frac{x}{R})$. Now
\begin{align*}
 & \, \int_{\R^N \times \R^N} \frac{|v_{R}(x)-v_{R}(y)|^p}{|x-y|^{N+sp}} \dxy \\  & \leq \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} \dxy+ \int_{\R^N \times \R^N} |u(y)|^p \frac{|\phi_{R}(x)-\phi_{R}(y)|^p}{|x-y|^{N+sp}} \dxy \\
 & := I_1 + I_2 \,.
\end{align*}
We estimate $I_2$ as follows.
\begin{align*}
I_2  & = \int_{\R^N} |u(y)|^p \int_{\R^N} \frac{|\phi_{R}(x)-\phi_{R}(y)|^p}{|x-y|^{N+sp}} \dxy \\
 & = \int_{\R^N} |u(y)|^p \int_{\R^N} \frac{|\phi_{R}(y+z)-\phi_{R}(y)|^p}{|z|^{N+sp}} \ \mathrm{d}z \mathrm{d}y  \\
  & \leq \int_{\R^N} |u(y)|^p |D^s \phi_{R}(y)|^p  \dy \\
  & = \frac{1}{R^{sp}} \int_{\R^N} |u(y)|^p \bigg|D^s \phi\bigg(\frac{y}{R}\bigg)\bigg|^p  \dy \ \ \  \mbox{\cite[Lemma \ 2.1]{Bonder}}  \\
  & \leq  \left( \int_{\R^N} |u(y)|^{p_s^*} \mathrm{d}y \right)^{\frac{N-sp}{N}} \left( \int_{\R^N} |D^s \phi(y)|^{\frac{N}{s}}   \mathrm{d}y  \right)^{\frac{sp}{N}} \\
  & \leq \|D^s \phi\|_{\infty}^p \left( \int_{\R^N} |u(y)|^{p_s^*}  \dy \right)^{\frac{N-sp}{N}} \left( \int_{\R^N} \left|\frac{D^s \phi(y)}{\|D^s \phi\|_{\infty}} \right|^{\frac{N}{s}}  \dy  \right)^{\frac{sp}{N}} \\
 & \leq \|D^s \phi\|_{\infty}^p \left( \int_{\R^N} |u(y)|^{p_s^*} \dy \right)^{\frac{N-sp}{N}} \left( \int_{\R^N} \left|\frac{D^s \phi(y)}{\|D^s \phi\|_{\infty}} \right|^{p}  \dy  \right)^{\frac{sp}{N}} \\ 
  & \leq C  \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} \dxy
  \ = \ C I_1 \ \ \mbox{[by Remark \ref{infestimate}]}.
  \end{align*}
  Therefore, the result follows.
\end{proof}
%{\color{red}Now we define the following closed subspace of $\mathcal{H}_{s,p}(\R^N)$:
%$$\mathcal{H}_{s,p,0}(\R^N)=\overline{C_c(\R^N)} \ \mbox{in} \ \mathcal{H}_{s,p}(\R^N).$$}
In the next proposition, we establish a necessary and sufficient condition for the weights $w\in L^1_{loc}(\mathbb{R}^N)$ to be in the space $\mathcal{H}_{s,p,0}(\R^N).$
\begin{proposition} \label{charF}
Let  {$0<s<1<p<\frac{N}{s}$ and} $w \in L^1_{loc}(\mathbb{R}^N)$. Then, $w \in \mathcal{H}_{s,p,0}(\R^N)$ if and only if for every $\epsilon >0$, there exists $w_{\epsilon} \in L^{\infty}(\R^N) $ such that $|Supp(w_{\epsilon})|< \infty$ (where $|E|$ denotes the $N$-dimensional Lebesgue measure of the set $E$) and $\norm{w-w_{\epsilon}}_{\mathcal{H}_{s,p}({\R^N})}< \epsilon.$ %  {still in some places it is missing, recheck }
\end{proposition}

\begin{proof}
Let $w \in \mathcal{H}_{s,p,0}(\R^N)$ and $\epsilon >0$ be given. By definition of $\mathcal{H}_{s,p,0}(\R^N)$, there exists $w_{\epsilon} \in C_c(\R^N)$ such that $\norm{w-w_{\epsilon}}_{\mathcal{H}_{s,p}(\mathbb{R}^N)} < \epsilon .$ This $w_{\epsilon}$ \tb{fulfills} our requirements. 
For the converse part, take a $w$ satisfying the hypothesis. Let $\epsilon >0 $ be arbitrary. Then there exists $w_{\epsilon} \in L^{\infty}(\R^N)$ such that 
$|Supp(w_{\epsilon})|< \infty$ and $\norm{w-w_{\epsilon}}_{\mathcal{H}_{s,p}(\R^N)}< \frac{\epsilon}{2}.$
Thus, $w_{\epsilon} \in L^{\frac{N}{sp}}(\R^N)$ and hence there exists $ \phi_{\epsilon} \in C_c^{}(\R^N)$ such that 
 $\norm{w_{\epsilon}-\phi_{\epsilon}}_{\frac{N}{sp}} < \frac{\epsilon}{2C}$,
 where $C$ is the embedding constant for the embedding $ L^{\frac{N}{sp}}(\R^N)$ into $\mathcal{H}_{s,p}(\R^N)$, \tb{see Proposition \ref{Lorentz space embedding} for a proof of this embedding}. Now by triangle inequality, we obtain $\norm{w-\phi_{\epsilon}}_{\mathcal{H}_{s,p}(\mathbb{R}^N)}< \epsilon$ as required.
\end{proof}

% \begin{remark}
% From the above calculation, it is clear that, if $u \in \mathcal{D}^{s,p}_0(\R^N)$ and $\Phi \in C_c^{\infty}(\R^N)$, then $v:=u\Phi \in \mathcal{D}^{s,p}_0(\R^N)$ and \begin{align}
%     \int_{\R^N \times \R^N} \frac{|v(x)-v(y)|^p}{|x-y|^{N+sp}} & \leq C_1 \int_{\R^N \times \R^N} |\Phi(x)|^p \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} dx dy \\ & \leq C_2 \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^p}{|x-y|^{N+sp}} dx dy.
% \end{align}
% \end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some important embeddings}
In this subsection, we will prove some important embedding results to help us reach our final goal later. First, we prove the following result:
 \begin{proposition} \label{Lorentz space embedding}
For  {$0<s<1<p<\frac{N}{s}$}, $L^{\frac{N}{sp}, \infty}(\mathbb{R}^{N})$ is continuously embedded in $\mathcal{H}_{s,p}(\mathbb{R}^{N})$.
\end{proposition}
\begin{proof}
Observe that $\mathrm{Cap}_{s,p}(F^{\star})  \leq \mathrm{Cap}_{s,p}(F)$. The inequality follows from P\'olya-Szeg\"o inequality  \cite[Theorem 9.2]{Almgren}. Also, we know that $\mathrm{Cap}_{s,p}(F^{\star}) \geq \mathcal{K}_{N,s,p} R^{N-sp},$ where R is the radius of $F^{\star}$ and $ \mathcal{K}_{N,s,p} > 0 $ is a constant independent of $R$ \cite[Theorem 3]{Xiao}. Now for a relatively compact set F, \[
\dfrac{\int_{F}|w|(x) \dx}{\mathrm{Cap}_{s,p}(F)} \leq \dfrac{\int_{F^{\star}} w^{\star}(x) \dx}{\mathrm{Cap}_{s,p}(F^{\star})} \leq \dfrac{\tb{\int_{0}^{\mu(F)} w^{\ast}(t) \dt}}{\mathcal{K}_{N,s,p} R^{N-sp}} = \dfrac{\omega_{N} R^{N} w^{\ast \ast}(\omega_{N} R^{N})}{\mathcal{K}_{N,s,p} R^{N-sp}} = \dfrac{R^{sp}~ w^{\ast \ast}(\omega_{N} R^{N})}{\mathcal{K}_{N,s,p}},
\]
where we use Hardy-Littlewood inequality \cite[Thoerem 3.2.10]{Edmunds} in the first and second inequality. By setting $\omega_{N}{R}^{N} = t,$ we get
\begin{eqnarray*}
\dfrac{\int_{F}|w|(x) \dx}{\mathrm{Cap}_{s,p}(F)} \leq {\mathcal{K}_{N,s,p}} \|w\|_{(\frac{N}{sp}, \infty)}.
\end{eqnarray*}
Now take the supremum over $F \Subset \R^N$ to obtain,
\begin{eqnarray*}
\|w\|_{\mathcal{H}_{s,p}(\R^N)} \leq {\mathcal{K}_{N,s,p}} \|w\|_{(\frac{N}{sp}, \infty)} \end{eqnarray*} %~\mbox{with} ~ \mathcal{K}_{N,s,p} > 0 ~\mbox{constant~depending~on}~N,s,p.
with $\mathcal{K}_{N,s,p} > 0$ and the constant is depending on $N,s$ and $p$.
\end{proof}
Let us define the following spaces % {lets change the notation as follows: $\mathcal{H}_{s,p}(\mathbb{R}^{N}) \hookrightarrow \mathcal{H}_{s,p}(\mathbb{R}^{N})$, $\mathcal{F}_{\frac{N}{sp}}(\mathbb{R}^{N}) \hookrightarrow L^{\frac{N}{sp},\infty}_0(\mathbb{R}^{N})$ and $\mathcal{H}_{s,p,0}(\mathbb{R}^{N}) \hookrightarrow \mathcal{H}_{s,p}_0(\mathbb{R}^{N})$} 
$$L^{\frac{N}{sp},\infty}_0(\mathbb{R}^{N}) = \overline{C_{c}^{}(\mathbb{R}^{N})} ~~\mbox{in} ~~L^{\frac{N}{sp},\infty}(\mathbb{R}^{N}),$$
$$\mathcal{H}_{s,p,0}(\mathbb{R}^{N}) =  \overline{C_{c}^{}(\mathbb{R}^{N})} ~~\mbox{in} ~~\mathcal{H}_{s,p}(\mathbb{R}^{N}).$$
\begin{proposition}
Let  {$0<s<1<p<\frac{N}{s}$}. Then $L^{\frac{N}{sp},\infty}_0(\mathbb{R}^{N}) \subset \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$.
\end{proposition}
\begin{proof}
\tb{Recall that} $L^{\frac{N}{sp},\infty}_0(\mathbb{R}^{N})$ is the closure of $C_{c}^{}(\mathbb{R}^{N})$ in $L^{\frac{N}{sp}, \infty}(\mathbb{R}^{N})$ and $\mathcal{H}_{s,p,0}(\mathbb{R}^{N})$ is the closure of $C_{c}^{}(\mathbb{R}^{N})$ in $\mathcal{H}_{s,p}(\mathbb{R}^{N})$. Now by Proposition \ref{Lorentz space embedding}, we have $\|\cdot\|_{\mathcal{H}_{s,p}(\R^N)} \leq C \|\cdot\|_{\frac{N}{sp}, \infty}$. Therefore, it is immediate that $L^{\frac{N}{sp},\infty}_0(\mathbb{R}^{N})$ is contained in $\mathcal{H}_{s,p,0}(\mathbb{R}^{N})$.
\end{proof}

In the following proposition, we establish the Lorentz-Sobolev embedding for $\D^{s,p}(\mathbb{R}^{N})$  {using the fractional Hardy-type inequality \eqref{Fractional Hardy}.}
\begin{proposition}
Let $p>1$ with $sp<N$, then $\D^{s,p}(\mathbb{R}^{N})$ is continuously embedded in the Lorentz space $L^{p^{*}_{s},p}(\mathbb{R}^{N})$, where $p^{*}_{s} = \frac{Np}{N-sp}.$
\end{proposition}
\begin{proof}
 Let $w \in \mathcal{H}_{s,p}(\mathbb{R}^{N})$ be such that $w^{\star} \in \mathcal{H}_{s,p}(\mathbb{R}^{N}).$ Then using the P\'olya-Szeg\"o inequality \cite[Theorem 9.2]{Almgren}, we have
\begin{eqnarray*}
\int_{\mathbb{R}^{N}} w^{\star} |u^{\star}|^{p} \dx &\leq & C \|w^{\star}\|_{\mathcal{H}_{s,p}(\R^N)} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u^{\star}(x) - u^{\star}(y)|^{p}}{|x-y|^{N+sp}} \dxy \\ 
 &\leq & C \|w^{\star}\|_{\mathcal{H}_{s,p}(\R^N)} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy,\ \forall u \in \D^{s,p}(\mathbb{R}^{N}).
\end{eqnarray*}
In Particular, for $w(x) = \dfrac{1}{\omega_{N}^{\frac{sp}{N}} |x|^{sp}},~w^{*}(t) = \dfrac{1}{t^{\frac{sp}{N}}},~\mbox{and}~ \|w^{\star}\|_{\mathcal{H}_{s,p}(\R^N)} \leq C(N,p,s).$ Also we have $$\int_{\mathbb{R}^{N}} w^{\star} |u^{\star}|^{p} \dx = \int_{0}^{\infty} w^{*}(t) |u^{*}(t)|^{p} \mathrm{d}t.$$ Thus, from the above inequality we have, 
\begin{eqnarray*}
 \int_{0}^{\infty} \dfrac{1}{t^{\frac{sp}{N}}} |u^{*}(t)|^{p} \mathrm{d}t&=& \int_{0}^{\infty} w^{*}(t) |u^{*}(t)|^{p} \mathrm{d}t = \int_{\mathbb{R}^{N}} w^{\star} |u^{\star}|^{p} \dx\\
 &\leq& C(N,p,s) \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy,\ \forall u \in \D^{s,p}(\mathbb{R}^{N}).
\end{eqnarray*}
 The left-hand side of the above inequality is $|u|^{p}_{(p^{*}_{s},p)}$, a quasi-norm equivalent to the norm $\|u\|^{p}_{(p^{*}_{s},p)}$ in $L^{p^{*}_{s},p}(\mathbb{R}^{N})$. This completes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Concentration compactness}
Let $\mathbb{M} (\R^N)$ be the space of all regular, finite,  Borel-signed measures on $\R^N.$ Then $\mathbb{M} (\R^N)$ is a Banach space with respect to the norm $\norm{\mu}=|\mu|(\R^N)$ (total variation of the measure $\mu$). By Riesz representation theorem, we know that $\mathbb{M}(\R^N)$ is the dual of $C_0(\R^N)$ (= $\overline{C_c(\R^N)}$ in $L^{\infty}(\R^N)$) \cite[Theorem 14.14, Chapter 14]{Border}. The next proposition follows from the uniqueness part of the Riesz representation theorem.
\begin{proposition} \label{defmeasure}
 Let $\mu \in \mathbb{M}(\R^N)$ be a positive measure. Then for an open $V \subseteq \R^N$,
 \[ \mu(V)= \sup \left \{ \int_{\R^N} \phi \, \dm : 0 \leq \phi \leq 1, \phi \in C_c^{\infty}(\R^N) \ with \ Supp(\phi) \subseteq V   \right \}\]
and for any Borel set $E \subseteq \R^N$, $\mu(E):= \inf \big\{ \mu(V) : E \subseteq V \ \mbox{and} \ V \text {is open } \big\}$.
\end{proposition}
A sequence $(\mu_n)$ is said to be weak* convergent to $\mu$ in $\mathbb{M}(\R^N)$, if
 \begin{eqnarray*}
  \int_{\R^N} \phi \, \dm_n \ra  \int_{\R^N} \phi\, \dm, \ as \ n \ra \infty,  \forall\,  \phi \in C_0(\R^N).
 \end{eqnarray*}
 In this case, we denote $\mu_n \wrastar \mu$. The following proposition is a consequence of the Banach-Alaoglu theorem \cite[Chapter 5, Section 3]{Conway}, which states that for any normed linear space $X$, the closed unit ball in  $X^*$ is weak* compact.
\begin{proposition} \label{BanachAlaoglu}
 Let $(\mu_n)$ be a bounded sequence in $\mathbb{M}(\R^N)$, then there exists $\mu \in \mathbb{M}(\R^N)$ such that $\mu_n \overset{\ast}{\rightharpoonup} \mu$ up to a subsequence.
\end{proposition}
\begin{proof}
 Recall that, if $X=C_0(\R^N)$ then by Riesz Representation theorem \cite[Theorem 14.14, Chapter 14]{Border} $X^*=\mathbb{M}(\R^N)$. Thus, the proof follows from the Banach-Alaoglu theorem \cite[Chapter 5, Section 3]{Conway}. 
\end{proof} 
For $u_n, u\in {\mathcal{D}^{s,p}(\R^N)}$ and a Borel set  $ E $ in   $\R^N,$ we  denote 
\begin{align*}
\nu_n(E)=\int_E w|u_n - u|^p \, \dx \,, &\,  \quad \Ga_n(E)=\int_E|D^s (u_n-u)|^p \, \dx \,  \\ 
\widetilde{\Ga}_n(E) &=\int_E|D^s u_n|^p \, \dx \,.
 \end{align*}
If $u_n\wra u$ in $\mathcal{D}^{s,p}(\R^N)$, then $\nu_n$, $\Ga_n$ and $\widetilde{\Ga}_n$ 
  have weak* convergent sub-sequences (Proposition \ref{BanachAlaoglu}) in $\mathbb{M}(\R^N)$. Let
   \[\nu_n \overset{\ast}{\rightharpoonup} \nu \,, \qquad \Gamma_n \overset{\ast}{\rightharpoonup} \Gamma \,, \qquad \widetilde{\Gamma}_n \overset{\ast}{\rightharpoonup} \widetilde{\Gamma} \  \mbox{ in } \mathbb{M}(\R^N).\] 
We develop a $w$-depended concentration compactness lemma using our concentration function $\C_w$ (see \eqref{cw} for the definition). Our results are analogous to the results of Tertikas \cite{Tertikas} and Smets \cite{Smets}. The following Lemma is due to \cite[Remark 2.5]{Bonder}.
\begin{lemma} \label{lem: 1}
Let $0<s<1<p<\frac{N}{s}$ and $\phi \in W^{1,\infty}(\R^N)$ with compact support.
Let $u_n \wra u$ in $\mathcal{D}^{s,p}(\R^N)$. Then
$$\displaystyle \lim_{n\ra \infty} \int_{\R^N} |(u_n-u)(x)|^p |D^s \phi|^p(x) \ \dx = 0 \,.$$
\end{lemma}
\begin{remark} \rm
Lemma \ref{lem: 1} also holds if we replace $\phi$ with  $\psi \in C_b^{\infty}(\R^N)$ with $0 \leq \psi \leq 1$, $\psi = 0$ on $B_1(0)$ and $\psi =1$ on $B_2(0)^c$. 
\end{remark}
\begin{corollary} \label{passing_limit}
Let  {$0<s<1<p<\frac{N}{s}$ and} $u_n \wra u$ in $\mathcal{D}^{s,p}(\R^N)$. Let $\phi \in W^{1,\infty}(\R^N)$ with compact support or $\phi \in C_b^{\infty}(\R^N)$ with $0 \leq \phi \leq 1$, $\phi = 0$ on $B_1(0)$ and $\phi =1$ on $B_2(0)^c$. Then, for $v_n=(u_n-u)\phi$, we have
\begin{align*}
 \tb{\overline{\lim_{n \ra \infty}}} \int_{\R^N \times \R^N} \frac{|v_n(x)-v_n(y)|^p}{|x-y|^{N+sp}} \dxy    \leq   \tb{\overline{\lim_{n \ra \infty}}} \int_{\R^N \times \R^N} |\phi(y)|^p\frac{|(u_n-u)(x)-(u_n-u)(y)|^p}{|x-y|^{N+sp}} \dxy  \,. 
\end{align*}
\end{corollary} 
\noi Next, we prove the absolute continuity of $\nu$ with respect to $\Gamma$. 
 \begin{lemma}\label{mlc1}
 Let  {$0<s<1<p<\frac{N}{s}$. Assume that} $w \in \mathcal{H}_{s,p}(\R^N) $, $w \geq 0$ and $u_n \wra u$ in $ \mathcal{D}^{s,p}(\R^N)$. Then for any Borel set $E$ in $\R^N$,
   \[\nu(E) \leq C_{H} \C^*_w \Gamma (E), \ \mbox{where $\C^*_w = \displaystyle\sup_{x \in \R^N} \C_w(x)$ } .\]
  \end{lemma}
  \begin{proof}
As $u_n \wra u$ in $ \mathcal{D}^{s,p}(\R^N)$, $u_n \ra u$ in $L^{p}_{loc}(\R^N)$.  For $\Phi \in C_c^{\infty}(\R^N)$, $(u_n-u) \Phi \in \D^{s,p}(\R^N)$. Thus, denoting $v_n=(u_n-u)\Phi$, we have
\begin{align*}
  \int_{\R^N} |\Phi|^p \ \mathrm{d} \nu_n  =  \int_{\R^N} w|(u_n-u)\Phi|^p \dx  \leq   C_H \norm{w}_{\mathcal{H}_{s,p}(\R^N)}  \int_{\R^N \times \R^N} \frac{|v_n(x)-v_n(y)|^p}{|x-y|^{N+sp}} \dxy  \,.
\end{align*}
Taking $n \ra \infty$ and using Corollary \ref{passing_limit}, we obtain
 \begin{align} \label{forrmk}
     \int_{\R^N} |\Phi|^p \ \mathrm{d} \nu \leq C_{H} \norm{w}_{\mathcal{H}_{s,p}(\R^N)} \int_{\R^N} |\Phi|^p \ \mathrm{d} \Gamma .
 \end{align}
Now by Proposition \ref{defmeasure}, we get 
  \begin{equation}\label{measureinequality1}
   \nu(E) \leq C_{H} \norm{w}_{\mathcal{H}_{s,p}(\R^N)} \Gamma (E),  \  \forall E \ \text{Borel in} \ \R^N.
  \end{equation}
 In particular, $\nu \ll \Gamma$ and hence by Radon-Nikodym theorem, 
 \begin{equation} \label{measureinequality}
  \nu(E) = \int_E  \frac{\mathrm{d} \nu}{\mathrm{d} \Gamma} \  \mathrm{d}\Gamma \ , \forall E \ \text{Borel  in} \ \R^N. 
 \end{equation}
 Further, by Lebesgue differentiation theorem (page 152-168 of \cite{Federer}), we have 
 \begin{equation} \label{Lebdiff}
  \frac{\mathrm{d} \nu}{\mathrm{d} \Gamma}(x) = \lim_{r \ra 0} \frac{\nu (B_r(x))}{\Gamma (B_r(x))}.
 \end{equation}
 Now replacing $w$ by $w \chi_{B_r(x)}$ and proceeding as before,
 \[ \nu(B_r(x)) \leq C_{H} \norm{w \chi_{B_r(x)}}_{\mathcal{H}_{s,p}(\R^N)} \ \Gamma (B_r(x)).\] 
 Thus from \eqref{Lebdiff} we get 
\begin{eqnarray} \label{21}
 \frac{\mathrm{d} \nu}{\mathrm{d} \Gamma} (x) \leq C_{H} \C_w(x)
\end{eqnarray} 
and hence 
$\norm{\frac{\mathrm{d} \nu}{\mathrm{d} \Gamma}}_{\infty} \leq C_{H} \C^*_w$. Now from \eqref{measureinequality} we obtain $\nu(E) \leq C_{H} \C^*_w \Gamma (E)$ 
for all Borel subsets $E$ of $\R^N$.
\end{proof}    
   
The next Lemma gives a lower estimate for the measure $\tilde{\Gamma}.$ Similar estimate is obtained in Lemma 2.1 of \cite{Smets}.  We make a weaker assumption, $\overline{\sum_w}$ is of Lebesgue measure $0$, than the assumption $\overline{\sum_w}$ is countable.
\begin{lem} \label{lemma9}
Let  {$0<s<1<p<\frac{N}{s}$ and} $w \in \mathcal{H}_{s,p}(\R^N)$ be such that $w \ge 0$ and $|\overline{\sum_w}|=0$. If $u_n \wra u$ in $ \D^{s,p}(\R^N)$, then 
\begin{equation*}
   \tilde{\Gamma} \geq \begin{cases}
     |D^s u|^p + \frac{\nu}{C_{H} \C_w^*}, \quad \text{if} \ \C_w^* \neq 0, \\
     |D^s u|^p, \quad \text{otherwise}.
    \end{cases}
\end{equation*}
\end{lem}
\begin{proof}
Our proof splits into three steps.\\
{\bf Step 1:} $\tilde{\Ga} \geq |D^s u|^p.$ \tb{As $u_n \wra u$ in $ \mathcal{D}^{s,p}(\R^N)$, $u_n \ra u$ a.e. in $\R^N$. Using Fatous lemma, one can see that $|D^s u| \leq \liminf_{n \ra \infty}  |D^s u_n|$ a.e. in $\R^N$. Now,  let $\phi \in C_c^{\infty}(\R^N)$ with $0\leq \phi \leq 1$, we need to show that
$\int_{\R^N} \phi \ \mathrm{d}\tilde{\Ga} \geq \int_{\R^N} \phi |D^s u|^p \, \dx. $
Notice that
\begin{align*}\int_{\R^N} \phi \, \mathrm{d}\tilde{\Ga}= \lim_{n \ra \infty} \int_{\R^N} \phi \, \mathrm{d}\tilde{\Ga}_n  = \lim_{n \ra \infty} \int_{\R^N} \phi |D^s u_n|^p \, \dx \geq \int_{\R^N} \phi |D^s u|^p \, \dx ,\end{align*}
where the last inequality follows from Fatous lemma.}
% \begin{align*}\int_{\R^N} \phi \, \mathrm{d}\tilde{\Ga}= \lim_{n \ra \infty} \int_{\R^N} \phi \, \mathrm{d}\tilde{\Ga}_n  = \lim_{n \ra \infty} \int_{\R^N} \phi |D^s u_n|^p \, \dx =
%  \lim_{n \ra \infty} \int_{\R^N} F(x,D^s u_n(x)) \, \dx ,\end{align*}
% where $F:\R^N \times \R \mapsto \R$ is defined as $F(x,z)=\phi(x)|z|^p.$ Clearly, $F$ is a Carath\'eodory function  and $F(x,.)$ is convex for almost every $x$. Hence, by 
% Theorem 2.6 of \cite{Fillip} (page 28), we have
% $\lim_{n \ra \infty} \int_{\R^N} \phi |D^s u_n|^p \, \dx \geq  \int_{\R^N} \phi |D^s u|^p \, \dx$ and this proves our claim 1.

\noi {\bf Step 2:} $\tilde{\Gamma}=\Gamma$, on $\overline{\sum_w}.$ Let $E\subset\overline{\sum_w}$ be a Borel set. Thus, for each $m \in \N$, there exists an open subset $O_{m}$ containing $E$ such that $|O_m|=|O_{m} \setminus E| < \frac{1}{m}$. Let $\var >0$ be given. Then, for any $\phi \in C_c^{\infty}(O_{m})$ with $0 \leq \phi \leq 1$, we have
\begin{align*}
    &\bigg|\int_{\R^N}  \phi \ \mathrm{d}\Gamma_n \, \dx  - \int_{\R^N}  \phi \ d\tilde{\Gamma}_n \, \dx\bigg| \\ 
    &= \left|\int_{\R^N}  \phi |D^s (u_n-u)|^p \, \dx -\int_{\R^N}  \phi |D^s u_n|^p \, \dx \right| \\
     &\leq  \int_{\R^N \times \R^N} \phi(x) \frac{\big| |u_n(x)-u_n(y)|^p - |(u_n-u)(x)-(u_n-u)(y)|^p \big|}{|x-y|^{N+sp}}\, \dxy \\
    &\leq  \epsilon \int_{\R^N \times \R^N} \phi(x) \frac{ |u_n(x)-u_n(y)|^p}{|x-y|^{N+sp}}\, \dxy  + c(\epsilon,p) \int_{\R^N \times \R^N} \phi(x) \frac{ |u(x)-u(y)|^p}{|x-y|^{N+sp}}\ \dxy \\
    & \leq \epsilon \int_{\R^N \times \R^N} \frac{ |u_n(x)-u_n(y)|^p}{|x-y|^{N+sp}}\, \dxy + c(\epsilon,p) \int_{O_m}  |D^s u|^p \, \dx \,.
\end{align*}
\tb{Now taking $n \rightarrow \infty$, we obtain $
 \left|\int_{\R^N}  \phi \, \mathrm{d}\Gamma  -\int_{\R^N}  \phi \, \mathrm{d}\tilde{\Gamma}  \right|  \leq  \epsilon L + c(\epsilon,p) \int_{O_{m}}   |D^s u|^p \ \dx
$, where $L=\sup_{n \in \N} \{\|u_n\|_{s,p}\} <\infty$.
Therefore,
\begin{eqnarray*} 
\left|\Gamma (O_m)-\tilde{\Gamma} (O_m) \right| \leq \epsilon L + c(\epsilon,p) \int_{O_{m}}   |D^s u|^p \, \dx \,.
\end{eqnarray*}
Thus, as $m \ra \infty,$ $|O_m|\ra 0$ and hence $| \Gamma (E)-\tilde{\Gamma} (E)| \leq \epsilon L $, where $\epsilon>0$ is arbitrary, i.e., $\Gamma(E)=\tilde{\Gamma} (E).$}

\noi {\bf{Step 3:}} $ \tilde{\Gamma} \geq |D^s u|^p + \frac{\nu}{C_{H} \C_w^*},$ if $\C_w^* \neq 0$. Let $\C_w^* \neq 0$. Then from Lemma \ref{mlc1} we have  $ \Gamma \geq \frac{\nu}{C_{H} \C_w^*}$. Furthermore, \eqref{21} and \eqref{measureinequality} ensures that $\nu$ is supported on $\sum_w.$ Hence Step 1 and Step 2 yields the following: 
\begin{equation}\label{rep1}
 \tilde{\Gamma} \geq \left\{\begin{array}{ll}
    |D^s u|^p,  &  \\
     \frac{\nu}{C_{H} \C_w^*} .
\end{array}\right.    
\end{equation}
Since $|\overline{\sum_w}|=0$, the measure $|D^s u|^p$ is supported inside $\overline{\sum_w}^{c}$ and hence from \eqref{rep1} we easily obtain  $\tilde{\Gamma} \geq |D^s u|^p +  \frac{\nu}{C_{H} \C_w^*}.$
\end{proof}
\noi Now we prove the following Lemma.
     \begin{lemma}\label{mlc2}
   Let  {$0<s<1<p<\frac{N}{s}$ and} $w \in \mathcal{H}_{s,p}(\R^N)$, $w \geq 0$ and $u_n \wra u$ in $\mathcal{D}^{s,p}(\R^N)$. Set
   \begin{eqnarray*}
    \nu_{\infty} = \displaystyle\lim_{R \ra \infty} \overline{\lim_{n \ra \infty}}  \nu_n( \overline{B_R}^c) \quad \mbox{and} \quad \Gamma_{\infty} =  \displaystyle\lim_{R \ra \infty} \overline{\lim_{n \ra \infty}}  \Gamma_n( \overline{B_R}^c).
   \end{eqnarray*} 
  Then
\begin{enumerate}[(i)]
 \item $\nu_{\infty} \leq C_{H} \C_w(\infty)  \Gamma_{\infty} \nonumber,$
  \item $ \displaystyle \overline{\lim}_{n \ra \infty} \int_{\R^N} w|u_n|^p\, \dx= \int_{\R^N} w|u|^p\, \dx+ \norm{\nu} + \nu_{\infty}$,
\item[(iii)] Further, if $|\overline{\sum_w}|=0$, then we have

\begin{equation*}
\displaystyle \overline{\lim}_{n \ra \infty} \int_{\R^N} |D^s u_n|^p \dx \geq \begin{cases}
 \int_{\R^N} |D^s u|^p \dx + \frac{\norm{\nu}}{C_H\C_w^*} +  \Gamma_{\infty}, \quad \ \text{if} \ \ \C_w^* \neq 0 \\
 \int_{\R^N} |D^s u|^p \dx  +  \Gamma_{\infty}, \quad \ \text{otherwise}. 
     \end{cases}
  \end{equation*}
\end{enumerate}
  \end{lemma}
\begin{proof}
(i) For $R>0$, choose $\Phi_R \in C_b^{1}(\R^N)$ satisfying  $0\leq \Phi_R \leq 1$, $\Phi_R = 0 $ on $\overline{B_R}$ and $\Phi_R = 1 $ on $B_{R+1}^c$. Clearly, $v_n:=(u_n-u) \Phi_R \in \mathcal{D}^{s,p}_0( \displaystyle\overline{B_R}^c)$. Since
$\norm{w \chi_{ \overline{B_R}^c}}_{\mathcal{H}_{s,p}(\R^N)} < \infty, $ by Maz'ya's theorem,
\begin{align}
& \, \int_{\R^N} |\Phi_R|^p \ \mathrm{d}\nu_n  =  \int_{\R^N} w|(u_n-u)\Phi_R|^p \ \dx  = \int_{\overline{B_R}^c} w |v_n|^p \ \dx \nonumber \\  & \leq C_H   \norm{w \chi_{\overline{B_R}^c}}_{\mathcal{H}_{s,p}(\R^N)}   \int_{\R^N \times \R^N} \frac{|v_n(x)-v_n(y)|^p}{|x-y|^{N+sp}} \ \dxy \nonumber \\
& \leq C_{H} \norm{w \chi_{\overline{B_R}^c}}_{\mathcal{H}_{s,p}(\R^N)} \int_{\R^N \times \R^N} |\Phi_R(x)|^p \frac{|(u_n-u)(x)-(u_n-u)(y)|^p}{|x-y|^{N+sp}} \ \dxy \nonumber \\
&= C_{H} \norm{w \chi_{\overline{B_R}^c}}_{\mathcal{H}_{s,p}(\R^N)} \int_{\R^N} |\Phi_R|^p \ \mathrm{d}\Gamma_n. \label{lab: 1} 
\end{align}
Also, notice that 
\begin{align*}
    \nu_n(\overline{B_{R+1}^c}) & \leq \int_{\R^N} |\Phi_R|^p \ \mathrm{d}\nu_n \leq \nu_n(\overline{B_{R}^c}), \, \\
    \Gamma_n(\overline{B_{R+1}^c}) & \leq \int_{\R^N} |\Phi_R|^p \ \mathrm{d}\Gamma_n \leq \Gamma_n(\overline{B_{R}^c}) \,.
\end{align*}
Thus,
\begin{equation} \label{nu infty gamma infty}
    \displaystyle\nu_{\infty}=\lim_{R \ra \infty} \overline{\lim_{n \ra \infty}} \int_{\R^N} |\Phi_R|^p \ \mathrm{d}\nu_n ~~\text{and}~~ \displaystyle\Gamma_{\infty}=\lim_{R \ra \infty} \overline{\lim_{n \ra \infty}}\int_{\R^N} |\Phi_R|^p \ \mathrm{d}\Gamma_n.
\end{equation}
Consequently, by taking $n \ra \infty$, and $R \ra \infty$ in \eqref{lab: 1}, we get $\nu_{\infty} \leq C_{H} \C_{w}(\infty) \Gamma_{\infty}.$
 
\noi $(ii)$ By choosing $\Phi_R$ as above and using Br\'ezis-Lieb lemma together with \eqref{nu infty gamma infty} we have
\begin{align*}
 \overline{\lim_{n\ra \infty}} \int_{\R^N} w| u_n|^p \dx
 &= \overline{\lim_{R\ra \infty}} \  \overline{\lim_{n\ra \infty}} \left[ \int_{\R^N} w| u_n|^p (1-\Phi_R)\dx + \int_{\R^N} w| u_n|^p \Phi_R \dx  \right] \\
&=\overline{\lim_{R\ra \infty}} \ \overline{\lim_{n\ra \infty}} \left[  \int_{\R^N} w| u|^p (1-\Phi_R)  \dx  + \int_{\R^N} w| u_n-u|^p (1-\Phi_R) \dx + \int_{\R^N} w| u_n|^p \Phi_R \dx \right]   \\
&= \int_{\R^N} w| u|^p \dx + \norm{\nu} + \nu_{\infty}. 
\end{align*} 
\noi $(iii)$  Notice that 
 \begin{align}
\overline{\lim_{n\ra \infty}} \int_{\R^N} |D^s u_n|^p \dx &= \overline{\lim_{n\ra \infty}} \left[ \int_{\R^N} |D^s u_n|^p (1-\Phi_R) \dx + \int_{\R^N} |D^s u_n|^p \Phi_R \dx\right] \nonumber \\ &= \tilde{\Gamma}(1-\Phi_R) \dx+ \overline{\lim_{n\ra \infty}}  \int_{\R^N}  \Phi_R \ \mathrm{d}\tilde{\Gamma}_n. \label{lab: 2}
  \end{align}
Now for a given $\epsilon>0$ we have, \begin{align*}
 &\,   \left|\int_{\R^N}   \Phi_R \, \mathrm{d}\Gamma_n \, \dx -\int_{\R^N}   \Phi_R \, \mathrm{d}\tilde{\Gamma}_n \, \dx \right| \\ &= \left|\int_{\R^N}   \Phi_R |D^s (u_n-u)|^p \, \dx -\int_{\R^N}   \Phi_R |D^s u_n|^p \, \dx \right| \\
   &\leq  \int_{\R^N \times \R^N} \Phi_R(x) \frac{\big| |u_n(x)-u_n(y)|^p - |(u_n-u)(x)-(u_n-u)(y)|^p \big|}{|x-y|^{N+sp}}\, \dxy \\
    &\leq  \epsilon \int_{\R^N \times \R^N} \Phi_R(x) \frac{ |u_n(x)-u_n(y)|^p}{|x-y|^{N+sp}}\, \dxy + c(\epsilon,p) \int_{\R^N \times \R^N} \Phi_R(x) \frac{ |u(x)-u(y)|^p}{|x-y|^{N+sp}}\, \dxy \\
    & \leq \epsilon \int_{\R^N \times \R^N} \frac{ |u_n(x)-u_n(y)|^p}{|x-y|^{N+sp}}\, \dxy + c(\epsilon,p) \int_{\overline{B_R}^c}  |D^s u|^p \, \dx \,.
\end{align*} 
As limit $n \ra \infty$ and $\epsilon \ra 0$, we get
\begin{align*}
    \left|\int_{\R^N}   \Phi_R \, \mathrm{d}\Gamma \ \dx -\int_{\R^N}   \Phi_R \, \mathrm{d}\tilde{\Gamma} \ \dx \right| \leq c(p) \int_{\overline{B_R}^c}  |D^s u|^p \, \dx \,.
\end{align*}
By taking $R \ra \infty$, we have $\Gamma_{\infty}=\displaystyle \lim_{R \ra \infty} \int_{\R^N}   \Phi_R \ \mathrm{d}\tilde{\Gamma} \ \dx=\displaystyle \lim_{R \ra \infty} \overline{\lim_{n \ra \infty}} \int_{\R^N}   \Phi_R \ \mathrm{d}\tilde{\Gamma}_n \ \dx$.
Therefore, by taking $R \ra \infty$ in \eqref{lab: 2}, we get
\begin{equation*} 
 \overline{\lim_{n\ra \infty}} \int_{\Om} |D^s u_n|^p \ \dx = \|\tilde{\Gamma}\|+ \Gamma_{\infty}.   
\end{equation*}
Now, using Lemma \ref{lemma9}, we obtain \begin{equation*}
\displaystyle \overline{\lim}_{n \ra \infty} \int_{\R^N} |D^s u_n|^p \ \dx \geq \begin{cases}
\displaystyle \int_{\R^N} |D^s u|^p \dx + \frac{\norm{\nu}}{C_H\C_g^*} +  \Gamma_{\infty}, \quad \ \text{if} \ \C_g^* \neq 0 \\
\displaystyle \int_{\R^N} |D^s u|^p \dx +  \Gamma_{\infty}, \quad \ \text{otherwise}. 
     \end{cases}
  \end{equation*} 
\end{proof} 

\subsection{Proof of Theorem \ref{allinone1}}
  {In this subsection, we  prove the equivalence given by Theorem \ref{allinone1}. We start with the following key lemma that gives a necessary condition for the compactness of $W$ on $\mathcal{D}^{s,p}(\R^N)$.}
 \begin{lem} \label{cpct}
 Let  {$0<s<1<p<\frac{N}{s}$ and} $w \in \mathcal{H}_{s,p}(\R^N)$ and $W(u):=\displaystyle\int_{\R^N} |w| |u|^p \dx$ on $\mathcal{D}^{s,p}(\R^N)$ is compact. Then, 
 \begin{enumerate}
  \item[(i)] if $(A_n)$ is a sequence of bounded measurable subsets such that $\chi_{A_n}$ decreases to $0,$ then $$\displaystyle \norm{w \chi_{A_n}}_{\mathcal{H}_{s,p}(\R^N)} \ra 0 \text{ as } n \ra \infty.$$
  \item[(ii)] $\norm{w \chi_{B_n^c}}_{\mathcal{H}_{s,p}(\R^N)} \ra 0$
  as $n \ra \infty$.
 \end{enumerate}
 \end{lem}
\begin{proof} $(i)$ Let $(A_n)$ be a sequence of bounded measurable subsets such that $\chi_{A_n}$ decreases to $0$. Suppose that,  $\norm{w \chi_{A_n}}_{\mathcal{H}_{s,p}(\R^N)} \nrightarrow 0$. Then, there exists $a>0$ such that $\norm{w \chi_{A_n}}_{\mathcal{H}_{s,p}(\R^N)} >a$, for all $n$ (by the monotonicity of the norm).
  Thus, there exists $F_n \Subset \R^N$ and $ u_n \in  \mathcal{N}_{s,p}(F_n)$ such that  
 \begin{equation} \label{convDp}
 \int_{\R^N} |D^s u_n|^p \dx < \frac{1}{a} \int_{F_n \cap A_n} |w| \dx \leq \frac{1}{a}\int_{|u_n| = 1} |w| |u_n|^{p_{s}^*} \dx \,.
 \end{equation}
 Since $A_n$'s are bounded and $\chi_{A_n}$ decreases to $0$, it follows that $|A_n| \ra 0$, as $n \ra \infty.$ Hence, we also have $\int_{F_n \cap A_n} |w| \ \dx \ra 0$ as $n \ra \infty$ (as $w \in L^1(A_1)$). 
 Hence from the above inequalities, $u_n \ra 0$ in $\mathcal{D}^{s,p}(\R^N)$. Now take $v_n=\frac{u_n^{\frac{p_{s}^*}{p}}}{\|u_n\|_{s,p}}$. Then, one can show that $(v_n)$ is bounded in $\mathcal{D}^{s,p}(\R^N)$ and  $v_n \ra 0$ a.e. because $\|v_n\|_p^p=\frac{\|u_n\|_{p_{s}^*}^{p_{s}^*}}{\|u_n\|_{s,p}^{p}} \leq C\|u_n\|_{s,p}^{p_{s}^*-p} \ra 0$ as $n\ra \infty$. Thus, $v_n \wra 0$ in $\mathcal{D}^{s,p}(\R^N)$.   By the compactness of $W$ we infer that $\lim_{n\ra \infty} \int_{\R^N} |w||v_n|^p\dx =0.$
 On the other hand,  
 \begin{eqnarray*}
  \int_{\R^N} |w| |v_n|^p\, \dx &=& \int_{\R^N}  \frac{|w| |u_n|^{p_{s}^*}}{ \norm{u_n}_{s,p}^p}\, \dx
   \geq  \int_{|u_n| = 1} \frac{|w| |u_n|^{p_{s}^*}}{ \norm{u_n}_{s,p}^p}\, \dx >a \,,
 % &>&   a 
 \end{eqnarray*}
which is a contradiction.

\noi $(ii)$ If  $\norm{w \chi_{B_n^c}}_{\mathcal{H}_{s,p}(\R^N)} \nrightarrow 0$, as $n \ra \infty,$ then there exists $F_n \Subset \R^N$ such that
   \begin{eqnarray*}
a < \frac{\int_{F_n \cap B_n^c}  |w|\, \dx}{\cp(F_n)} \leq \frac{\int_{F_n \cap B_n^c} |w|\, \dx}{\cp(F_n \cap B_n^c)} 
\leq \frac{C\int_{F_n \cap B_n^c} |w|\, \dx}{\cp(F_n \cap B_n^c, \overline{B}_{\frac{n}{2}}^c) }
\end{eqnarray*}
 for some $a>0$ and $C>0$. The last inequality follows from part $(ii)$ of Proposition \ref{propofcap}.
 Thus, for each $n\in \N$ there exists $z_{n} \in \D^{s,p}_0( \overline{B}_{\frac{n}{2}}^c)$ with $z_n \geq 1$ on $F_n \cap B_n^c$ such that 
\[ \int_{\R^N} |D^s z_n|^p\, \dx < \frac{C}{a} \int_{F_n \cap B_n^c} |w| \,\dx \leq \frac{C}{a} \int_{\R^N} |w||z_n|^p\, \dx.\]
 By taking $v_n=\displaystyle \frac{z_n}{\norm{z_n}_{s,p}}$ and following a same argument as in $(i)$ we contradict the compactness of $W$.
\end{proof} 
Next   for $\phi \in C_c^{}(\R^N)$ we compute $\C_{\phi}$. For that, we will be using the fact that
$$\cp((F \cap B_r)^{\star}) \geq \mathcal{K}_{N,s,p} r^{N-sp} \,,$$
where $\mathcal{K}_{N,s,p}>0$ is a constant independent of $r$ \cite{Jie}.
 \begin{proposition} \label{Cgzero}
  Let $\phi \in C_c(\R^N)$. Then $\C_{\phi} \equiv 0.$
 \end{proposition}
 \begin{proof}
 First notice that, for $\phi \in C_c^{}(\R^N),$
\begin{eqnarray*} 
  \norm{\phi \chi_{B_r(x)}}_{\mathcal{H}_{s,p}(\R^N)} =  \sup_{F \Subset \R^N} \left[ \frac{\int_{F \cap B_r(x)}|\phi|\dx}{\cp(F, \R^N)}\right]  
 \leq  \sup_{F \Subset \R^N} \left[ \frac{ \sup (|\phi|) |(F\cap B_r)^{\star}|}{\cp((F \cap B_r)^{\star})}  \right]. \nonumber
 \end{eqnarray*}
 The last inequality follows from P\'olya-Szeg\"o inequality \cite[Theorem 9.2]{Almgren}.
 If $d$ is the radius of $(F \cap B_r)^{\star}$ then
 \[\frac{ |(F\cap B_r)^{\star}|}{\cp((F \cap B_r)^{\star})} \leq \text{C}(N,s,p) \frac{d^N}{d^{(N-sp)}} = \text{C}(N,s,p) d^{sp} \leq \text{C}(N,s,p) r^{sp} .\]
 Thus, $\C_{\phi}(x) = \lim_{r \ra 0} \norm{\phi \chi_{B_r(x)}}_{\mathcal{H}_{s,p}(\R^N)} =0 $. Also, one can easily see that $\C_{\phi}(\infty)=0 $ as $\phi$  has compact support.
 \end{proof}
 

Now, we prove our main theorem. 
 %\begin{theorem}
 %\label{allinone}
 % Let $w \in \mathcal{H}_{s,p}(\R^N)$. Then the following statements are equivalent:
 % \begin{enumerate}
%   \item[(i)] $W:\mathcal{D}^{s,p}_0(\mathbb{R}^N) \to \R $ is compact,
%   \item[(ii)] $w$ has absolute continuous norm in $\mathcal{H}_{s,p}(\R^N)$,
 %  \item[(iii)] $w \in \mathcal{H}_{s,p,0}(\R^N)$,
 %  \item[(iv)] $\C^*_w =0= \C_w(\infty)$.
 % \end{enumerate}
 % \end{theorem}
\begin{proof}[Proof of Theorem \ref{allinone1}]
 $(i) \implies (ii):$ Let $W$ be compact. Take a sequence of measurable subsets $(A_n)$ 
 of $\R^N$ such that $\chi_{A_n}$ decreases to $0$ a.e. in $\R^N$. Part $(ii)$ of Lemma \ref{cpct} gives $\norm{w \chi_{B_n^c}}_{\mathcal{H}_{s,p}(\R^N)} \ra 0$, as $n \ra \infty$. Choose $\epsilon >0$ arbitrarily. There exists $N_0 \in \N,$ 
such that $\norm{w \chi_{B_n^c}}_{(\R^N)} \leq \frac{\epsilon}{2},$ for all $n \geq N_0.$ Now $A_n= (A_n \cap B_{N_0}) \cup (A_n \cap B_{N_0}^c)$,  for each $n$. Thus, 
\[\norm{w \chi_{A_n}}_{\mathcal{H}_{s,p}(\R^N)} \leq \norm{w \chi_{A_n \cap B_{N_0}}}_{\mathcal{H}_{s,p}(\R^N)} + \norm{w \chi_{A_n \cap B_{N_0}^c}}_{\mathcal{H}_{s,p}(\R^N)} \leq \norm{w \chi_{A_n \cap B_{N_0}}}_{\mathcal{H}_{s,p}(\R^N)} + \frac{\epsilon}{2}.\]
 Part $(i)$ of Lemma \ref{cpct} implies that there exists a natural number $N_1(\geq N_0)$ such that $$\norm{w \chi_{A_n \cap B_{N_0}}}_{\mathcal{H}_{s,p}(\R^N)} \leq \frac{\epsilon}{2}, \ \forall n \geq N_1 \,,$$ and hence $\norm{w \chi_{A_n}}_{\mathcal{H}_{s,p}(\R^N)} \leq \epsilon$ for all $n \geq N_1$. 
 Therefore, $w$ has an absolutely continuous norm.

\noi $(ii) \implies (iii):$ Let $w$ has absolute continuous norm in $\mathcal{H}_{s,p}(\R^N)$. Then, $\norm{w \chi_{B_m^c}}_{\mathcal{H}_{s,p}(\R^N)} $ converges to $0$ as $m \ra \infty$. Let $\epsilon >0$ be arbitrary. We choose $m_{\var} \in \N$ such that $\norm{w \chi_{B_m^c}}_{\mathcal{H}_{s,p}(\R^N)} < \epsilon$, for all $m \geq m_{\var}$. Now for any $n \in \N$,
\[w = w \chi_{\{|w| \leq n\} \cap B_{m_{\var}}} + w \chi_{\{|w| >n\} \cap B_{m_{\var}}} + w \chi_{B_{m_{\var}}^c} := w_n + z_n.\]
where $w_n=w \chi_{\{|w| \leq n\} \cap B_{m_{\var}}}$ and $z_n=w \chi_{\{|w| >n\} \cap B_{m_{\var}}} + w \chi_{B_{m_{\var}}^c}.$ Clearly, $w_n \in L^{\infty}(\R^N)$ and $|Supp(w_n)| < \infty $. 
Furthermore,
\[ \norm{z_n}_{\mathcal{H}_{s,p}(\R^N)} \leq \norm{w \chi_{\{|w| >n\} \cap B_{m_{\var}}}}_{\mathcal{H}_{s,p}(\R^N)} + \norm{w \chi_{B_{m_{\var}}^c}}_{\mathcal{H}_{s,p}(\R^N)} <  \norm{w \chi_{\{|w| >n\} \cap B_{m_{\var}}}}_{\mathcal{H}_{s,p}(\R^N)} + \epsilon \,. \]
 Now, $w \in L^1_{loc}(\R^N)$ ensures that $\chi_{\{|w| >n\} \cap B_{m_{\var}}} \ra 0$ as $n\ra \infty$. As $w$ has absolutely continuous norm, $\norm{w \chi_{\{|w| >n\} \cap B_{{m_{\var}}}}}_{\mathcal{H}_{s,p}(\R^N)} < \epsilon$ for large $n$. Therefore, $\norm{z_n}_{\mathcal{H}_{s,p}(\R^N)}< 2\epsilon$ for large $n$.
 Hence, Lemma \ref{charF} concludes that $w \in \mathcal{H}_{s,p,0}(\R^N)$.
 
 \noi $(iii) \implies (iv):$ Let $w \in \mathcal{H}_{s,p,0}(\R^N)$ and $\epsilon >0$ be arbitrary. Then there exists $w_\var \in C_c(\R^N)$ such that
 $\norm{w-w_\var}_{\mathcal{H}_{s,p}(\R^N)} < \epsilon$. Thus Proposition \ref{Cgzero} infers that $\C_{w_\var}$ vanishes.
Now as $w = w_\var + (w-w_\var)$, it follows that $\C_w(x) \leq \C_{w_\var}(x) + \C_{w - w_\var}(x) \leq \norm{w - w_\var}_{\mathcal{H}_{s,p}(\R^N)} < \epsilon$ and hence $\C^*_w=0$. By a similar argument one can show $\C_w(\infty)=0.$

\noi $(iv) \implies (i):$ Assume that $\C^*_w =0= \C_w(\infty)$. Let $(u_n)$ be a bounded sequence in $ \mathcal{D}^{s,p}(\R^N)$. Then by Lemma \ref{mlc2}, up to a sub-sequence we have,
 \begin{eqnarray*}
 \nu_{\infty} &\leq& C_H\ \C_w(\infty)  \Gamma_{\infty} \label{1},\\
 \norm{\nu} &\leq& C_H \C^{*}_w \norm{\Gamma} \label{2}, \\
 \tb{\lim_{n \ra \infty}} \int_{\R^N} |w||u_n|^p \dx &=& \int_{\R^N} |w||u|^p \dx + \norm{\nu} + \nu_{\infty} \label{3}.
 \end{eqnarray*}
 As $\C^*_w=0= \C_w(\infty)$ we immediately conclude that
 $\displaystyle \tb{\lim_{n \ra \infty}} \int_{\R^N} |w||u_n|^p\, \dx = \int_{\R^N} |w||u|^p\,\dx $
 and hence $W: \mathcal{D}^{s,p}(\R^N) \mapsto \R$ is compact.
 \end{proof} 
\section{Weighted Eigenvalue Problem} \label{WEVP}
This section deals with the weighted eigenvalue problem given by \eqref{Weighetd eigenvalue problem}. We show the existence of the first eigenvalue by using   {variational techniques on the} Rayleigh quotient and then prove some qualitative properties of the first eigenvalue. Finally, we prove  {the existence of infinitely many eigenvalues that increase to infinity.} 
% {\color{red}
% Our aim is to deal with the following fractional $p$-Laplacian eigenvalue problem :
% \begin{equation} \label{Weighetd eigenvalue problem}
%     (-\Delta_{p})^{s}u = \lambda w(x) |u|^{p-2}u ~~\text{in}~\mathbb{R}^{N},
% \end{equation}  where $0<s<1<p<\infty,~N>sp$ and $(-\Delta_{p})^{s}$ is the fractional $p$-Laplacian operator defined by
% $$(-\Delta_{p})^{s}u = 2 \lim_{\epsilon \rightarrow 0^{+}} \int_{\mathbb{R}^{N} \backslash B_{\epsilon}(x)} \frac{|u(x) - u(y)|^{p-2}(u(x)-u(y))}{|x-y|^{N+sp}}dy~~\text{for}~x \in \mathbb{R}^{N},$$ where $B_{\epsilon}(x) = \{ y \in \mathbb{R}^{N} ~:~ |x-y| < \epsilon \}.$ The weight function $w = w_{1} - w_{2}~\text{with}~ w_{1},w_{2} \geq 0,$ is such that  $ w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$ and $w_{2} \in L^{1}_{loc}(\mathbb{R}^{N})$. The space $\mathcal{H}_{s,p,0}(\mathbb{R}^{N})$ is the closure of $C_{c}^{\infty}(\mathbb{R}^{N})$ in $\mathcal{H}_{s,p}(\mathbb{R}^{N})$.\\
% By an eigenvalue of (\ref{Weighetd eigenvalue problem}) we mean $\lambda \in \mathbb{R}$ such that, (\ref{Weighetd eigenvalue problem}) admits a non-zero weak solution in $D^{s,p}(\mathbb{R}^{N})$; i.e., there exists  $u \in D^{s,p}(\mathbb{R}^{N}) \backslash \{0\}$ such that for all $v \in D^{s,p}(\mathbb{R}^{N})$, we have
% \begin{equation} \label{Lagrange equation}
%      \iint_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p-2} (u(x)-u(y)) (v(x) -v(y))}{ |x-y|^{N+sp}} \,dxdy = \lambda \int_{\mathbb{R}^{N}} w|u|^{p-2}uv~dx. 
% \end{equation}
% The function $u$ satisfying \eqref{Lagrange equation} is an eigenfunction corresponding to the eigenvalue $\lambda$. If one of the eigenfunctions corresponding to $\lambda$ is of constant sign, then we say that $\lambda$ is a principal eigenvalue. The eigenvalue $\lambda$ is called simple if all the eigenfunctions corresponding to $\lambda$ are unique up to constant multiples.
% \begin{theorem} \label{Infinite eigenvalue}
%  Assume that $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$ and $w_{2} \in L_{loc}^{1}(\mathbb{R}^{N})$ with $w_{1} \not\equiv 0$, then there exists a sequence of eigenvalues $\{ \lambda_{k} \}$ for the problem (\ref{Weighetd eigenvalue problem}) such that $$ 0< \lambda_{1} < \lambda_{2} \leq \lambda_{3} \leq ... \leq \lambda_{k} \leq ...., ~~~~ \lambda_{k} \rightarrow \infty ~~\text{as} ~~k \rightarrow \infty.$$ The first eigenvalue $\lambda_{1}$ is simple and the eigenfunction corresponding to $\lambda_{1}$ may be positive in $\mathbb{R}^{N}$.
% \end{theorem}
% }

\subsection{Qualitative behaviour of the first eigenvalue}
We show the existence of an eigenvalue by following a direct variational approach. We begin with the Rayleigh quotient $Q(u)$ given by
% We use a direct variational method for the existence of an eigenvalue. For that we consider the following Rayleigh quotient 
\begin{equation} \label{Rayleigh quotient}
   Q(u) = \dfrac{\int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}}\, \dxy}{\int_{\mathbb{R}^{N}} w|u|^{p}\, \dx},
\end{equation}
with the domain of definition 
\begin{equation} \label{L}
    \mathbb{L}:= \{ u \in \D^{s,p}(\mathbb{R}^{N}): \int_{\mathbb{R}^{N}} w|u|^{p}\, \dx > 0 \} \,.
\end{equation}
Since $w \in L_{loc}^{1}(\mathbb{R}^{N})$ and $w_{1} \not\equiv 0$, then by \cite[Proposition 4.2]{Prashanth} there exists $\phi \in C_{c}^{\infty}(\mathbb{R}^{N})$ such that $\int_{\mathbb{R}^{N}} w|\phi|^{p}dx >0$. Therefore, the set $\mathbb{L}$ is non-empty.
% \tr{mention here why $\mathbb{L}$ is non-empty.}
Now, let us consider 
\begin{equation} \label{M}
  \mathbb{S} := \{ u \in \D^{s,p}(\mathbb{R}^{N}) : \int_{\mathbb{R}^{N}} w|u|^{p}\, \dx = 1 \},
\end{equation}
\begin{equation} \label{J(u)}
%   J(u) = \frac{1}{p} \iint_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}} dxdy.
 J(u) =  \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}}\, \dxy.
\end{equation}
 Suppose $Q$ is $C^{1}$. In that case, the critical points of $Q$ over $\mathbb{L}$ correspond to the Euler-Lagrange equation associated with the weighted eigenvalue problem (\ref{Weighetd eigenvalue problem}), and the corresponding critical values of $Q$ are the eigenvalues of the problem (\ref{Weighetd eigenvalue problem}).  Observe that finding a critical point of the Rayleigh quotient $Q$ over the domain $\mathbb{L}$ is similar to finding the critical point of the functional $J$ over $\mathbb{S}$, i.e., there is a one-to-one correspondence between them. Therefore, we try to find the critical points of the functional $J$ on $\mathbb{S}$ by employing some sufficient  {conditions} on $w_1$. One of the main difficulties in showing the existence of a critical point of $J$ on $\mathbb{S}$ arises due to the non-compactness of the map $W$. Since we have a weak assumption on $w_{2}$, i.e., it is just locally integrable, therefore the map $W: \D^{s,p}(\mathbb{R}^{N}) \rightarrow \mathbb{R}$ given by
\begin{equation} \label{W(u)}
% W(u) = \frac{1}{p}\int_{\mathbb{R}^{N}} w|u|^{p}\dx.
W(u) = \int_{\mathbb{R}^{N}} w|u|^{p}\,\dx,
\end{equation}
may not even be continuous and hence $\mathbb{S}$ may not be closed in $\D^{s,p}(\mathbb{R}^{N})$. Despite that, we prove that a sequence of minimizers of $J$ on $\mathbb{S}$ has a weak limit, which also lies in $\mathbb{S}$. From the definition of the space $\D^{s,p}(\mathbb{R}^{N})$, it is easy to check that the functional $J$ becomes coercive and weakly lower semi-continuous on $\D^{s,p}(\mathbb{R}^{N})$. Further, if $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$, the map $W_{1}: \D^{s,p}(\mathbb{R}^{N}) \rightarrow \mathbb{R}$ given by
\begin{equation} \label{W1(u)}
W_{1}(\varphi) = \int_{\mathbb{R}^{N}} w_{1}|\varphi|^{p}\,\dx,
\end{equation}
is compact on $\D^{s,p}(\mathbb{R}^{N})$ by Theorem \ref{allinone1}.

\begin{theorem}
Let $w \in L_{loc}^{1}(\mathbb{R}^{N})$ with $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N}), w_1 \not\equiv 0$ and $sp<N$. Then $J$ admits a minimizer on $\mathbb{S}$.
\end{theorem}

\begin{proof}
Since $w \in L_{loc}^{1}(\mathbb{R}^{N})$ and $w_{1} \not\equiv 0$, then by \cite[Proposition 4.2]{Prashanth} there exists $\phi \in C_{c}^{\infty}(\mathbb{R}^{N})$ such that $\int_{\mathbb{R}^{N}} w|\phi|^{p}dx >0$
 and hence $\mathbb{S} \neq \emptyset$. Let $\{u_{n}\}$ be a minimizing
sequence for $J$ on $\mathbb{S}$; i.e.,
    \begin{equation*}
    \lim_{n \rightarrow \infty} J(u_{n}) = \lambda_{1} := \inf_{u \in \mathbb{S}} J(u).
    \end{equation*}
By the coercivity of $J$, $\{u_{n}\}$ is bounded in $\D^{s,p}(\mathbb{R}^{N}) $ and hence by reflexivity of $\D^{s,p}(\mathbb{R}^{N})$, the sequence $\{u_{n}\}$ admits a weakly convergent subsequence in $\D^{s,p}(\mathbb{R}^{N})$. Let us denote the subsequence by $\{u_{n}\}$ itself and the weak limit by $u$ in $\D^{s,p}(\mathbb{R}^{N})$. Further, the compactness of the map $W_{1}$ gives
     \begin{equation*}
    \lim_{n \rightarrow \infty} \int_{\mathbb{R}^{N}} w_{1}|u_{n}|^{p}\,\dx = \int_{\mathbb{R}^{N}} w_{1}|u|^{p}\,\dx.
     \end{equation*}
Since $u_{n} \in \mathbb{S}$, we write 
     \begin{equation*}
    \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p}\,\dx = \int_{\mathbb{R}^{N}} w_{1}|u_{n}|^{p}\,\dx -1.
     \end{equation*}
Also, we know that the embedding $\D^{s,p}(\mathbb{R}^{N}) \hookrightarrow L_{loc}^{p}(\mathbb{R}^{N})$ is compact, thus $u_{n} \rightarrow u$ a.e. in $\mathbb{R}^{N}$ up to a subsequence. We apply Fatou's Lemma to get
     \begin{equation*}
    \int_{\mathbb{R}^{N}} w_{2}|u|^{p}\,\dx \leq \int_{\mathbb{R}^{N}} w_{1}|u|^{p}\,\dx -1,
     \end{equation*}
which shows that $ \int_{\mathbb{R}^{N}} w|u|^{p}\dx \geq 1$. Setting $\tilde{u} := \dfrac{u}{(\int_{\mathbb{R}^{N}} w|u|^{p}\,\dx )^{1/p}}$, and since $J$ is weakly lower semi-continuous, we have 
    \begin{equation*}
    \lambda_{1} \leq J(\Tilde{u}) = \dfrac{J(u)}{\int_{\mathbb{R}^{N}} w|u|^{p}\, \dx} \leq J(u) \leq \liminf_{n} J(u_{n}) = \lambda_{1}.
    \end{equation*}
Thus the equality must hold at each step and $\int_{\mathbb{R}^{N}} w|u|^{p}\dx =1 $, which shows that $u \in \mathbb{S}$ and $ J(u) = \lambda_{1}$. Hence, $J$ admits a minimizer $u$ on $\mathbb{S}$.
\end{proof}
Further, we prove that any minimizer of $Q$ on $\mathbb{L}$ is an eigenfunction of \eqref{Weighetd eigenvalue problem}.
% Note that $Q$ is not sufficiently regular to conclude that \tr{$u$?}  is an eigenfunction of (\ref{Lagrange equation}) corresponding to $\lambda_{1}$ using critical point theory.
\begin{proposition} \label{u is a eigenfunction}
Let $u$ be a minimizer of $Q$ on $\mathbb{L}$. Then $u$ is an eigenfunction of (\ref{Weighetd eigenvalue problem}).
\end{proposition}
\begin{proof}
For each $\phi \in C_{c}^{\infty}(\mathbb{R}^{N})$, we can verify that $Q$ admits directional derivative along $\phi$ by using dominated convergence theorem. It is given that $u$ is a minimizer of $Q$ on $\mathbb{L}$, therefore we have a necessary condition
      \begin{align*}
    \dfrac{\mathrm{d}}{\mathrm{d}t} Q(u + t \phi) |_{t = 0} &= 0.\end{align*} 
   This further implies 
   \begin{align*} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p-2} (u(x)-u(y)) (\phi(x) -\phi(y))}{ |x-y|^{N+sp}}\, \dxy &= \lambda_{1} \int_{\mathbb{R}^{N}} w|u|^{p-2}u\phi\,\dx, 
     \end{align*}
     $\text{for all}~\phi \in C_{c}^{\infty}(\mathbb{R}^{N})$. Now using the density of $ C_{c}^{\infty}(\mathbb{R}^{N})$ into $\D^{s,p}(\mathbb{R}^{N})$, we can conclude
    \begin{equation*}
    \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p-2} (u(x)-u(y)) (\phi(x) -\phi(y))}{ |x-y|^{N+sp}}\, \dxy = \lambda_{1} \int_{\mathbb{R}^{N}} w|u|^{p-2}u\phi\,\dx, 
    \end{equation*}
    $\text{for all}~ \phi \in \D^{s,p}(\mathbb{R}^{N}).$
\end{proof}
Next, we prove that the first eigenfunction does not change its sign. We adapt the idea from the article \cite{Cui} to prove this Lemma. 
\begin{lemma} \label{Positive}
The first eigenfunctions (i.e., the eigenfunctions corresponding to the first eigenvalue $\lambda_1$) of the weighted eigenvalue problem (\ref{Weighetd eigenvalue problem}) are of a constant sign. Moreover, a non-negative first eigenfunction is positive.
\end{lemma}
\begin{proof}
We consider $u_{1}$ the first eigenfunction of \eqref{Weighetd eigenvalue problem} corresponding to the first eigenvalue $\lambda_1$. Then $u_1$ is a minimizer of $J$ over $\mathbb{S}$. Since $u_1 \in \mathbb{S}$, this implies that $|u_1|\in \mathbb{S}$. Now we have
\begin{align*}
    \lambda_1 = \inf\limits_{u \in \mathbb{S}} \int_{\R^N \times \R^N} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}}\,\dxy &\leq \int_{\R^N \times \R^N} \frac{\big||u_1(x)|-|u_1(y)|\big|^{p}}{|x-y|^{N+sp}}\,\dxy \\
    &\leq \int_{\R^N \times \R^N} \frac{|u_1(x)-u_1(y)|^{p}}{|x-y|^{N+sp}}\,\dxy = \lambda_1,
\end{align*}
% which implies that $|u_1|$ is also an eigenfunction corresponding to the eigenvalue $\lambda_1$. \tr{Thus it remains true if we consider the eigenfunction $u_1$ as a non-negative function i.e. $u_1 \geq 0$}  {what do u mean?}. 
Therefore, equality must hold at each step, which implies either $u_{1}^{+} \equiv 0$ or $u_{1}^{-} \equiv 0$. Thus, the eigenfunction $u_{1}$ corresponding to the first eigenvalue $\lambda_1$ does not change its sign.
% Further, there is a one-to-one correspondence between the minimizers of $J$ over $\mathbb{S}$ and the minimizers of $Q$ over $\mathbb{L}$. If we assume $u_1 \geq 0$. Then by Proposition \ref{u is a eigenfunction}, $u_{1}$ also solves (\ref{Weighetd eigenvalue problem}) in the weak sense i.e.
%  \begin{equation*}
%      (-\Delta_{p})^{s}u_{1} - \lambda_{1} w (u_{1})^{p-1} = 0 ~~\text{in}~ \mathbb{R}^{N}.
%  \end{equation*}
 If we assume $u_1 \geq 0$, then we have
\begin{equation*}
     (-\Delta_{p})^{s}u_{1} + \lambda_{1}w_{2} (u_{1})^{p-1} = \lambda_{1}w_{1} (u_{1})^{p-1} \geq 0 ~~\text{in}~\mathbb{R}^{N}.
 \end{equation*}
Thus the strong minimum principle \cite[Theorem 1.2]{Pezzo} yields $u_{1} >0$ a.e. in $\mathbb{R}^{N}$.
% It is clear that the eigenfunctions corresponding to $\lambda_{1}$ are the minimizers of $Q$ on $\mathbb{L}$. Let $u$ be a minimizer of $Q$ on $\mathbb{L}$. Since $u = u_{1} - u_{2} \not\equiv  0$ either $u_{1} ~\text{or}~u_{2}$ is non zero. Without loss of generality, we may assume that $u_{1} \not\equiv 0$. Now by taking $u_{1}$ as a test function in (\ref{Lagrange equation}), we see that $u_{1}$ also minimizes $Q$ on $\mathbb{L}$. Thus by Proposition \ref{u is a eigenfunction}, $u_{1}$ also solves (\ref{Weighetd eigenvalue problem}) in the weak sense i.e.
%  \begin{equation*}
%      (-\Delta_{p})^{s}u_{1} - \lambda_{1} w (u_{1})^{p-1} = 0 ~~\text{in}~ \mathbb{R}^{N}.
%  \end{equation*}
%  In particular, we have the following differential inequality in the sense of distributions:
% \begin{equation*}
%      (-\Delta_{p})^{s}u_{1} + \lambda_{1}w_{2} (u_{1})^{p-1} = \lambda_{1}w_{1} (u_{1})^{p-1} \geq 0 ~~\text{in}~\mathbb{R}^{N}.
%  \end{equation*}
% Moreover, it follows from the strong minimum principle \cite[Theorem 1.2]{Pezzo}, that $u_{1} >0$ a.e. in $\mathbb{R}^{N}$ and hence $u = u_{1}$.
\end{proof}
The following Lemma shows that the first eigenfunctions are the only eigenfunctions that do not change their sign.
We use the idea of \cite[Theorem 3.3]{Goyal2018eigenvalues} to prove the following Lemma.
\begin{lem}
The eigenfunctions of \eqref{Weighetd eigenvalue problem} corresponding to the eigenvalues other than $\lambda_1$ change its sign.
\end{lem} 
\begin{proof}
We assume that $u_1$ and $u$ are the eigenfunctions associated with two {distinct} eigenvalues $\lambda_1$ and $\lambda$, respectively. Then we have the following:
\begin{align}
     (-\Delta_{p})^{s}u_{1} &= \lambda_{1}w (u_{1})^{p-1} ~~\text{in}~(\D^{s,p}(\mathbb{R}^{N}))', \label{equation first}\\
      (-\Delta_{p})^{s}u_{} &= \lambda_{}w |u_{}|^{p-2}u ~~\text{in}~(\D^{s,p}(\mathbb{R}^{N}))'. \label{equation second}
\end{align}
We proceed by the method of contradiction. On the contrary, assume that the eigenfunction $u$ does not change its sign. Without the loss of generality, we may suppose that $u \geq 0$. We take $\{\phi_m\}$ as a sequence in $C^\infty_c(\mathbb{R}^{N})$ such that $\phi_m \rightarrow u_1$ {in $\D^{s,p}(\R^N)$} as $m \rightarrow \infty$. Now we take two test functions $w_1 = u_1,\  w_2 = \frac{\phi^p_m}{\left(u+\frac{1}{m}\right)^{p-1}}$. First we show that $w_2 \in \D^{s,p}(\mathbb{R}^{N})$. We have
\begin{align*}
    |w_2(x)-w_2(y)| &= \bigg|\frac{\phi^p_m(x)}{(u+\frac{1}{m})^{p-1}(x)} - \frac{\phi^p_m(y)}{(u+\frac{1}{m})^{p-1}(y)} \bigg|\\
    & = \bigg|\frac{\phi^p_m(x)- \phi^p_m(y)}{(u+\frac{1}{m})^{p-1}(x)} + \frac{\phi^p_m(y) \bigg((u+\frac{1}{m})^{p-1}(y) - (u+\frac{1}{m})^{p-1}(x) \bigg)}{(u+\frac{1}{m})^{p-1}(x)(u+\frac{1}{m})^{p-1}(y)} \bigg|\\
    & \leq m^{p-1}|\phi^p_m(x)- \phi^p_m(y)| + \norm{\phi_m}_{\infty}^p \frac{\big|(u+\frac{1}{m})^{p-1}(x) - (u+\frac{1}{m})^{p-1}(y) \big|}{(u+\frac{1}{m})^{p-1}(x)(u+\frac{1}{m})^{p-1}(y)}\\
    & \leq m^{p-1}p(\phi^{p-1}_m(x)+ \phi^{p-1}_m(y))|\phi_m(x)- \phi_m(y)|\\
    &\qquad + \norm{\phi_m}_{\infty}^p (p-1)\frac{\big((u+\frac{1}{m})^{p-2}(x) + (u+\frac{1}{m})^{p-2}(y)\big)}{(u+\frac{1}{m})^{p-1}(x)(u+\frac{1}{m})^{p-1}(y)}\times \\ &\qquad \quad \times\bigg|(u+\frac{1}{m})^{}(x) - (u+\frac{1}{m})^{}(y)\bigg|\\
    & \leq 2pm^{p-1}\norm{\phi_m}_{\infty}^{p-1}|\phi_m(x)- \phi_m(y)| + \norm{\phi_m}_{\infty}^p (p-1)|u(x) -u(y)| \times\\
    &\qquad \times \bigg( \frac{1}{(u+\frac{1}{m})(x)~(u+\frac{1}{m})^{p-1}(y)} +\frac{1}{(u+\frac{1}{m})^{p-1}(x)~(u+\frac{1}{m})(y)}  \bigg).\end{align*}
    Therefore, we finally get from the above: 
    \[ |w_2(x)-w_2(y)|  \leq C(m,p,\norm{\phi_m}_{\infty}) \big(|\phi_m(x)- \phi_m(y)| + |u(x) -u(y)| \big).\]
    Since $\phi_m, u \in \D^{s,p}(\mathbb{R}^{N})$, we can conclude from the above inequality that $w_2 \in \D^{s,p}(\mathbb{R}^{N})$. Taking $w_1$ and $w_2$ as test functions in \eqref{equation first} and \eqref{equation second} respectively, we have
\begin{equation} \label{equation third}
    \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u_1(x)-u_1(y)|^{p}}{ |x-y|^{N+sp}}\, \dxy = \lambda_{1} \int_{\mathbb{R}^{N}} w|u_1|^{p}\, \dx,
\end{equation} and
\begin{align} \label{equation sp}
\begin{split}
    \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p-2} (u(x)-u(y))}{ |x-y|^{N+sp}}\left(\frac{\phi^p_m(x)}{(u+\frac{1}{m})^{p-1}(x)}-\frac{\phi^p_m(y)}{(u+\frac{1}{m})^{p-1}(y)} \right)\, \dxy \\
    = \lambda_{} \int_{\mathbb{R}^{N}} w|u|^{p-2}u\frac{\phi^p_m(x)}{(u+\frac{1}{m})^{p-1}(x)}\,\dx.
\end{split}
\end{align}
From Lemma \ref{Picone identity} we have $K(\phi_m, u + \frac{1}{m}) \geq 0$, {where $K$ is as in \eqref{def:K}}. Now, combining this inequality with \eqref{equation sp}, we get
\begin{equation} \label{equation four}
    \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|\phi_m(x)-\phi_m(y)|^{p}}{ |x-y|^{N+sp}} \dxy  - \lambda_{} \int_{\mathbb{R}^{N}} w\phi_m^{p}\left(\frac{u}{u+ \frac{1}{m}} \right)^{p-1}\, \dx \geq 0.
\end{equation}
Next, subtracting \eqref{equation third} from \eqref{equation four} and taking the limit as $m \rightarrow \infty$, we obtain
\[(\lambda_1 -\lambda) \int_{\mathbb{R}^{N}}w |u_1|^p\, \dx \geq 0.\]
% As $u_1$ is the eigenfunction associated with the eigenvalue $\lambda_1$ and $u_1 \in \mathbb{S}$ \tr{at the beginning itself you choose $u_1$ like this, then u use that fact here}, we have $$\int_{\mathbb{R}^{N}}w |u_1|^p\, \dx=1.$$ 
Therefore, the above inequality holds if and only if $\lambda_1 > \lambda$ and a contradiction arises to the fact that $\lambda_1$ is the smallest eigenvalue. Thus, the proof is complete.
\end{proof}
{Further, we show the simplicity of the first eigenvalue of \eqref{Weighetd eigenvalue problem}.}
\begin{lemma} \label{Simple}
The eigenfunction of (\ref{Weighetd eigenvalue problem}) corresponding to $\lambda_{1}$ are unique up to some constant multiplication, i.e., $\lambda_{1}$ is simple.
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Let $\phi_{1}$ and $\phi_{2}$ be two eigenfunctions corresponding to the same eigenvalue $\lambda_{1}$, then we may suppose that $\phi_{1}$,~$\phi_{2}>0$ and $\phi_{1}, \phi_{2} \in \mathbb{S}$, namely,
\begin{equation*}
    \int_{\mathbb{R}^{N}} w|\phi_{1}|^{p} \dx = \int_{\mathbb{R}^{N}} w|\phi_{2}|^{p} \dx = 1.
\end{equation*}
Let 
\begin{equation*}
    \Phi = \bigg(\dfrac{\phi_{1}^{p}+\phi_{2}^{p}}{2}\bigg)^{1/p},
\end{equation*}
then we have $\Phi \in \mathbb{S}$. Since the function $\alpha(r,s) := |r^{1/p} - s^{1/p}|^{p}$ is convex for $r,s>0$, we have the following inequality
\begin{equation*}
    \alpha\bigg(\frac{r_{1}+r_{2}}{2}, \frac{s_{1}+s_{2}}{2}\bigg) \leq \frac{1}{2}\alpha(r_{1},s_{1}) + \frac{1}{2}\alpha(r_{2},s_{2}) ,
\end{equation*}
where the equality holds only for $r_{1}s_{2} = r_{2}s_{1}$ {(see \cite[Lemma 13]{Lindgren2014})}. 
% \tr{the blue sentence does not seem to be correct grammatically; looks incomplete}
Therefore, according to the above inequality and $\phi_{1},\phi_{2},\Phi \in \mathbb{S}$ we deduce,
\begin{align*}
    \lambda_{1} \leq \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|\Phi(x) - \Phi(y)|^{p}}{|x-y|^{N+sp}}\, \dxy \leq \frac{1}{2}\int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|\phi_{1}(x) - \phi_{1}(y)|^{p}}{|x-y|^{N+sp}}\,\dxy
    + \frac{1}{2} \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|\phi_{2}(x) - \phi_{2}(y)|^{p}}{|x-y|^{N+sp}}\dxy = \lambda_{1} \,. 
\end{align*}
Thus, equality must hold at each step. Therefore, $\phi_{1}(x)\phi_{2}(y) = \phi_{1}(y)\phi_{2}(x)$ which implies that $\phi_{1}(x) = c \phi_{2}(x)$ with $c \in \mathbb{R}$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Infinite set of eigenvalues}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{This section deals with the existence of an infinite set of eigenvalues of (\ref{Weighetd eigenvalue problem}). We
follow the Ljusternik-Schnirelmann theory on $C^1$-manifold due to Szulkin \cite{Szulkin}. The Ljusternik-Schnirelmann theory enables us to find the critical points of a functional $J$ on a manifold $M$. First, we recall the definition of the Palais-Smale (PS) condition and genus. Assume that $M$ is a $C^1$-manifold and $f \in C^{1}(M; \mathbb{R})$. A sequence $\{u_n\} \subset M$ is said to be a (PS) sequence on $M$ if $\{f(u_n)\}$ is bounded and $f'(u_n) \rightarrow 0$, where $f'(u)$ represents the Fr\'echet differential of $f$ at $u$. If every (PS) sequence $\{u_n\}$ admits a convergent subsequence, then we say $f$ satisfies the (PS) condition on $M$. Let $\Theta$ be the family of sets $A \subset M \setminus \{0\}$ such that $A$ is closed in $M$ and symmetric concerning $0$, i.e. $z \in A$ implies $-z \in A$. If $A \in \Theta$, then the Krasnoselski genus of $A$ is denoted by
$\gamma(A)$ and is defined as the smallest integer $k$ for which there exists a non-vanishing
odd continuous mapping from A to $\mathbb{R}^{k}$. When no such map exists for any $k$, we set $\gamma(A) = \infty$, and also we set $\gamma(\emptyset) = 0$.  We
refer to \cite{Rabinowitz} for more details and properties of the genus. We can deduce the next theorem from \cite[Corollary 4.1]{Szulkin}.}
\begin{theorem} \label{Ljusternik}
Let M be a closed symmetric $C^1$-submanifold of a real Banach space X and $0 \notin M$. Let $f \in C^1(M; \R)$ be an even function satisfying the (PS) condition
on M and is bounded below. Define
\[ \lambda_{j} := \inf_{A \in \Gamma_{j}} \sup_{x \in A} f(x),\]
where $\Gamma_j = \{ A \subset M : A ~\text{is compact and symmetric about origin},~ \gamma(A) \geq j\}$. If for a given $j,~ \lambda_j = \lambda_{j+1}= .~ .~ . = \lambda_{j+p} \equiv \lambda, ~then ~\gamma(K_\lambda) \geq p + 1,~ where~ K_\lambda = \{x \in M : f(x) = \lambda ,~ f'(x) = 0 \}$.
\end{theorem}
\noi It can be noticed that the set $ \mathbb{S} = \{ u \in \mathcal{D}^{s,p}(\mathbb{R}^{N}): \int_{\mathbb{R}^{N}} w|u|^{p} \dx = 1 \}$ may not admit a manifold structure from the topology on $\mathcal{D}^{s,p}(\mathbb{R}^{N})$, due to the weak assumptions on $w_{2}$. However, the set $\mathbb{S}$ inherits a $C^{1}$ Banach manifold structure from the following subspace $X$ of  $\mathcal{D}^{s,p}(\mathbb{R}^{N})$.

\noi For $w_{2} \in L^{1}_{loc}(\mathbb{R}^{N})$, we define
\[ \|u\|_{X}^{p} : = \|u\|_{s,p}^p + \int_{\mathbb{R}^{N}} w_{2}|u|^{p} \dx, \] and
\[ X:= \{ u \in  \mathcal{D}^{s,p}(\mathbb{R}^{N}): \|u\|_{X} < \infty\}. \]
% The following Lemma is motivated by \cite[Lemma 2.1]{Cui}, and the proof follows almost the same approach.
\begin{lemma}
The space $X = (X, \|\|_{X})$ is a uniformly convex Banach space.
\end{lemma}
\begin{proof} We break the proof into a few steps by using the approach as done in \cite[Lemma 5.1]{Chen2022}.\\
\noi {\bf Step 1:} First, we claim that $X$ is a complete space concerning the given norm. Let $\{u_{n}\}$ be a Cauchy sequence in $X$, i.e. given any $\epsilon > 0$, there exists a positive integer $N_0$ depending on $\epsilon$ such that if $n,m \geq N_0$, then 
\begin{equation} \label{Cauchy}
    \|u_{n} - u_{m}\|_{X} < \epsilon.
\end{equation}
Following the definition of the norm on $X$, we observe that $\|u_{n}-u_{m}\|_{s,p} \leq \|u_{n}-u_{m}\|_{X}< \epsilon.$ This implies that the sequence $\{u_{n}\}$ is Cauchy in $\D^{s,p}(\mathbb{R}^{N})$. By the completeness, there exists $u \in \D^{s,p}(\mathbb{R}^{N})$ such that $u_{n} \rightarrow u$ in $\D^{s,p}(\mathbb{R}^{N})$. Now, we need to show that $u \in X$. There exists a subsequence $\{u_{n_{k}}\}$ of $\{u_n\}$ such that $u_{n_{k}} \rightarrow u$ a.e. in $\mathbb{R}^{N}~\text{as}~k \rightarrow \infty$. Now, applying Fatou's Lemma and using (\ref{Cauchy}), we 
\begin{align*}
    \int_{\mathbb{R}^{N}} w_{2}|u|^{p} \dx \leq \liminf_{k \rightarrow \infty} \int_{\mathbb{R}^{N}} w_{2}|u_{n_{k}}|^{p} \dx \hspace{60mm}\\
    \leq \liminf_{k \rightarrow \infty} ( \|u_{n_{k}}- u_{N_0}\|_{X} + \|u_{N_0}\|_{X})^{p} \leq (\epsilon + \|u_{N_0}\|_{X})^{p} < \infty.
\end{align*}
Thus, $u \in X$. Further for $n \geq N_0$, we have $ \|u_{n}-u\|_{X} \leq \liminf_{k \rightarrow \infty}\|u_{n}-u_{n_{k}}\| \leq \epsilon$. Therefore, the sequence $\{u_n\}$ converges to $u$ strongly in $X$, i.e. $X$ is a complete space. \\
{\bf Step 2:} Now we want to show that $X$ is a uniformly convex Banach space. For $0 <\epsilon \leq 2$, let $u,v \in X$ such that 
\begin{align} \label{UC}
    \|u\|_{X}=1=\|v\|_{X} \ \text{and} \ \|u-v\|_{X} \geq \epsilon.
\end{align}
We prove the case $1<p<2$ and $p \geq 2$ separately. First, we begin with the case when $p \geq 2$. {Let us recall the following inequality \cite[Lemma 2.37, page 42]{Adams2003sobolev} given by}
\begin{equation} \label{adam}
    \bigg| \frac{a+b}{2} \bigg|^{p} + \bigg|\frac{a-b}{2} \bigg|^{p} \leq \frac{|a|^{p}+|b|^{p}}{2}, \ \text{for }a,b \in \mathbb{R}.
\end{equation}
From \eqref{adam}, we can deduce the following:
\begin{align*}
   \bigg\| \frac{u+v}{2} \bigg\|_{X}^{p} + \bigg\|\frac{u-v}{2} \bigg\|_{X}^{p} &=  \bigg\|{\frac{u+v}{2}}\bigg\|_{s,p}^{p} + \bigg\|{\frac{u-v}{2}}\bigg\|_{s,p}^{p} + \int_{\mathbb{R}^{N}} w_{2} \bigg(\bigg| \frac{u+v}{2}  \bigg|^{p} + \bigg| \frac{u-v}{2}  \bigg|^{p} \bigg) \dx\\
    &\leq \frac{1}{2} \bigg[  \|u\|_{s,p}^{p} + \|v\|_{s,p}^{p} + \int_{\mathbb{R}^{N}} w_{2} (|u|^{p}+ |v|^{p}) \dx \bigg]  \\
   & = \frac{1}{2} [\|u\|_{X}^{p} + \|v\|_{X}^{p}] = 1. 
\end{align*}
Thus by choosing $\delta = 1- \big(1-\big(\frac{\epsilon}{2}\big)^p\big)^{1/p}>0$, we can deduce from above that $\big\| \frac{u+v}{2} \big\|_{X} \leq 1-\delta$.
Therefore, the space $X$ is uniformly convex for $p \geq 2$.\\
\noi Now we consider the case when $1<p<2$. If we set $p'=\frac{p}{p-1}$, then by using \cite[Theorem 2.13, page 28]{Adams2003sobolev} and \cite[Lemma 2.37, page 42]{Adams2003sobolev}  for $u,v \in \D^{s,p}(\R^N)$ we have
\begin{align*}
    \bigg\| \frac{u+v}{2} \bigg\|_{s,p}^{p'} + \bigg\| \frac{u-v}{2} \bigg\|_{s,p}^{p'} &= \bigg\| \bigg( \bigg| \frac{u(x)+v(x)}{2} - \frac{u(y)+v(y)}{2} \bigg|  |x-y|^{\frac{-N-sp}{p}} \bigg)^{p'} \bigg\|_{L^{p-1}(\R^{2N})} \\
    & \qquad  + \bigg\| \bigg( \bigg| \frac{u(x)-v(x)}{2} - \frac{u(y)-v(y)}{2} \bigg|  |x-y|^{\frac{-N-sp}{p}} \bigg)^{p'} \bigg\|_{L^{p-1}(\R^{2N})} \\
    & \leq \bigg\| \bigg( \bigg| \frac{u(x)-u(y) + v(x)-v(y)}{2} \bigg|^{p'} + \bigg| \frac{u(x)-u(y) - (v(x)-v(y))}{2} \bigg|^{p'} \bigg)  \\ &\qquad  |x-y|^{\frac{-N-sp}{p-1}} \bigg\|_{L^{p-1}(\R^{2N})}\\
    & \leq \bigg\| \bigg(  \frac{|u(x)-u(y)|^p + |v(x)-v(y)|^p}{2} \bigg)^{\frac{1}{p-1}}  |x-y|^{\frac{-N-sp}{p-1}} \bigg\|_{L^{p-1}(\R^{2N})} \\
    & = \left[ \frac{1}{2} \|u\|_{s,p}^p + \frac{1}{2} \|v\|_{s,p}^p \right]^{\frac{1}{p-1}}.
\end{align*}
%\tr{"Remove the dots used for multiplication"}
Now for $0<\epsilon_1 \leq 2$ and $u,v \in \D^{s,p}(\R^N)$ such that $\|u\|_{s,p} = 1 = \|v\|_{s,p}$ and $\|u-v\|_{s,p} \geq \epsilon_1$, we can choose $\delta_1 = 1- \big( 1- (\epsilon_1 /2)^{p'} \big)^{\frac{1}{p'}}>0$ so that $ \big\| \frac{u+v}{2} \big\|_{s,p} \leq 1 - \delta_1$. Thus $\|\cdot\|_{s,p}$ is a uniformly convex norm. In a similar way, $\|u\|_{w_2,p} := \big( \int_{\R^N} w_2 |u|^p \dx \big)^{1/p}$ is also a uniformly convex norm. \\
From \eqref{UC}, we can notice that $\|u\|_{s,p} \leq 1$ and $\|v\|_{s,p} \leq 1$ and also we can assume that $\|u-v\|_{s,p} \geq \frac{\epsilon}{2^{1/p}}$. Further, we claim that there exists some $\delta_2 >0$ such that 
\begin{align} \label{E1}
    \bigg\|\frac{u+v}{2} \bigg\|_{s,p}^p \leq \frac{1- \delta_2}{2} \big(\|u\|_{s,p}^p + \|v\|_{s,p}^p \big). 
\end{align}
We prove the above claim by the method of contradiction. We break the proof into two parts.\\
\noi \textbf{Case 1}. Let $\|u\|_{s,p} = 1$ and $\|v\|_{s,p} \leq 1$. On contrary, we suppose that the claim \eqref{E1} is not true i.e., there must exist an $\epsilon_0 >0$ and two sequences $\{u_n\}$ and $\{v_n\}$ in $X$ such that $\|u_n\|_{s,p} = 1$ and $\|v_n\|_{s,p} \leq 1$ and $\|u_n-v_n\|_{s,p} \geq \frac{\epsilon_0}{2^{1/p}}$, and satisfying 
\begin{align} \label{E2}
    \bigg\|\frac{u_n+v_n}{2} \bigg\|_{s,p}^p \geq \frac{1}{2} \left(1- \frac{1}{n} \right) \left(\|u_n\|_{s,p}^p + \|v_n\|_{s,p}^p \right).
\end{align}
First we prove $\lim\limits_{n \rightarrow \infty} \|v_n\|_{s,p} =1$. If we suppose that $\lim\limits_{n \rightarrow \infty} \|v_n\|_{s,p} <1$, then by definition there exists a subsequence $\{v_{n_l}\}$ of $\{v_{n}\}$ such that $\|v_{n_l}\|_{s,p} \leq B <1$. Thus, we use the triangle inequality to obtain
\begin{align} \label{E3}
    \bigg\|\frac{u_{n_l}+v_{n_l}}{2} \bigg\|_{s,p}^p \leq \left(\frac{\|u_{n_l}\|_{s,p} + \|v_{n_l}\|_{s,p}}{2} \right)^p \leq \frac{\|u_{n_l}\|_{s,p}^p + \|v_{n_l}\|_{s,p}^p}{2}  \left[\left(\frac{1+B}{2} \right)^p \bigg/ \left(\frac{1+B^p}{2} \right) \right],
\end{align}
%\tr{"Remove the dots used for multiplication"}
where the last inequality follows by monotonicity (increasing) of the function $f(x) = \frac{(1+x)^p}{1+x^p},\ 1<p<2, \ x \in (0,1)$. Observe that $\big(\frac{1+B}{2} \big)^p \big/ \big(\frac{1+B^p}{2} \big)<1$ for all $1<p<2$. Therefore, a contradiction to \eqref{E2} arises by \eqref{E3}. Hence, we have $\lim\limits_{n \rightarrow \infty} \|v_n\|_{s,p} =1$. \\
We define $w_n = \frac{v_n}{\|v_n\|_{s,p}}$, then it is easy to observe that $\lim\limits_{n \rightarrow \infty}\|v_n - w_n\|_{s,p}=0$. Taking limit as $n \rightarrow \infty$ in \eqref{E2} and using $\lim\limits_{n \rightarrow \infty} \|v_n\|_{s,p} =1$, we have
\begin{align*} 
   1 \leq \lim\limits_{n \rightarrow \infty} \bigg\|\frac{u_{n}+v_{n}}{2} \bigg\|_{s,p} \leq \lim\limits_{n \rightarrow \infty}\bigg\|\frac{u_{n}+w_{n}}{2} \bigg\|_{s,p} \leq 1,
\end{align*}
which implies $\lim\limits_{n \rightarrow \infty}\big\|\frac{u_{n}+w_{n}}{2} \big\|_{s,p}=1$. Using the fact that $\|u_n-v_n\|_{s,p} \geq \frac{\epsilon_0}{2^{1/p}}$ for all $n\geq 1$, $\exists$ a positive integer $N_1$ such that $\|u_n-w_n\|_{s,p} \geq \frac{\epsilon_0}{2^{1+1/p}}$ for all $n \geq N_1$. Thus, the uniform convexity of the $\|\cdot\|_{s,p}$ norm ensures the existence of a $\delta_3 >0$ depending on $\epsilon_0$ such that $\big\|\frac{u_{n}+w_{n}}{2} \big\|_{s,p}\leq 1 - \delta_3$ for all $n \geq N_0$. This contradicts to $\lim\limits_{n \rightarrow \infty}\big\|\frac{u_{n}+w_{n}}{2} \big\|_{s,p}=1$. Hence, the claim \eqref{E1} follows.\\
\noi \textbf{Case 2}.  Let $\|u\|_{s,p} \leq 1$ and $\|v\|_{s,p} \leq 1$. Now either $\|u\|_{s,p} \leq \|v\|_{s,p}$ or $ \|u\|_{s,p} \geq \|v\|_{s,p}$. We assume that $\|u\|_{s,p} \geq \|v\|_{s,p}>0$ and the other case will follow similarly. We define $ u_1 = \frac{u}{\|u\|_{s,p}}, \ v_1 = \frac{v}{\|u\|_{s,p}} $. Notice that $\|u_1\|_{s,p}=1, \ \|v_1\|_{s,p}\leq 1 \ \text{and} \ \|u_1 - v_1\|_{s,p} \geq \frac{\epsilon}{2^{1/p}}$. By Case 1, the inequality \eqref{E1} is true for $u_1$ and $v_1$, and therefore \eqref{E1} also holds for $u$ and $v$.\\
Thus, using $\frac{\|u\|_{s,p}^p +\|v\|_{s,p}^p}{2} \geq \|\frac{u-v}{2} \|_{s,p}^p \geq \frac{\epsilon^p}{2^{p+1}}$, we get
\begin{align*}
    \left\|\frac{u+v}{2} \right\|_{X} &= \left(\left\|\frac{u+v}{2} \right\|_{s,p}^{p} + \int_{\R^N} w_2 \left|\frac{u+v}{2}\right|^p \dx \right)^{1/p} \\
    & \leq \left( (1- \delta_2)\frac{\|u\|_{s,p}^p +\|v\|_{s,p}^p}{2} + \int_{\R^N} w_2 \left( \frac{|u|^p+|v|^p}{2} \right) \dx \right)^{1/p} \\
    & = \left( \frac{1}{2} \|u\|_{X}^p + \frac{1}{2} \|v\|_{X}^p -\delta_2\frac{\|u\|_{s,p}^p +\|v\|_{s,p}^p}{2} \right)^{1/p} \\
    & \leq \left( 1 -\delta_2 \frac{\epsilon^p}{2^{p+1}} \right)^{1/p} := 1 - \delta,
\end{align*} 
where $\delta = 1- \left( 1 -\delta_2 \frac{\epsilon^p}{2^{p+1}} \right)^{1/p}>0$. Hence, we conclude that the space $(X, \|\cdot\|_X)$ is also uniformly convex for $1<p<2$.
\end{proof}
To fix the notations, let us denote the dual space of $X$ by $X'$ and the duality action by $\langle \cdot , \cdot \rangle$.
%  \tr{It is easy to observe that the functional $J$ given by
% \[  J(u) = \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}} \dxy, ~\forall u \in  \D^{s,p}(\mathbb{R}^{N}).\]
% belongs to $C^1(\mathbb{S}, \mathbb{R})$. It is an even function as well as bounded below by $0$.}
By the definition of $\|\cdot\|_{X}$, one can verify easily that the function $W_{2}$ given by
\[W_{2}(\varphi) = \int_{\mathbb{R}^{N}} w_{2}|\varphi|^{p} \dx ,\]
is continuous on $X$. Moreover, the map $W_{2}$ is continuously differentiable on $X$ and the Fr\"{e}chet derivative of $W_2$ is given by
\[\langle W'_{2}(\varphi), v \rangle =  p \int_{\mathbb{R}^{N}} w_{2}|\varphi|^{p-2} \varphi v\, \dx. \]
Similarly, using the fractional Hardy-type inequality, we can verify that the map $W_1$ is $C^1$ in $X$ and the Fr\"{e}chet derivative is given by
\[\langle W'_{1}( \varphi), v \rangle =  p \int_{\mathbb{R}^{N}} w_{1}| \varphi|^{p-2} \varphi v~ \dx. \] 
Thus for $w_1 \in \mathcal{H}_{s,p,0}(\R^N) \text{ and } w_2 \in L^{1}_{loc}(\R^N)$, the map $W$ is in $C^{1}(X;\R)$ and the Fr\"{e}chet derivative is given by
\[\langle W'_{}(\varphi), v \rangle =  p \int_{\mathbb{R}^{N}} w_{}| \varphi|^{p-2}\varphi v~ \dx. \] 
It is easy to note that for $u \in \mathbb{S},\  \langle W'(u), u \rangle = p$ and therefore the map $W'(u) \neq 0$. Thus, $1$ is a regular value of $W$. We say a real number $\alpha \in \R$ a regular value of $W$, if $W'(\varphi) \neq 0$ for all $\varphi$ such that $W(\varphi)=\alpha$. Moreover, the set $\mathbb{S}$ admits a $C^1$ Banach sub-manifold structure on $X$ by \cite[Example 27.2]{Deimling1985}.\\
Further, we verify that the functional $J$ satisfies all the conditions of Theorem \ref{Ljusternik}.
\begin{lemma}
The functional J is a $C^1$ on $\mathbb{S}$ and the Fr\"{e}chet derivative of J is given by $$\langle J'(u),v \rangle = p \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \dfrac{|u(x)-u(y)|^{p-2} (u(x)-u(y)) (v(x) -v(y))}{ |x-y|^{N+sp}} \dxy .$$
We omit the proof as it is straightforward.
\end{lemma}
\begin{remark}\label{rem2}
We can deduce from \cite[Proposition 6.4.35]{Drabek} that
\[ \|J'(u)\| = \min_{\lambda \in \mathbb{R}} \| J'(u) - \lambda W'(u)\| . \]
Thus $ J'(u_n) \rightarrow 0$  if and only if there exists a sequence $\{\lambda_n \}$ of real numbers such that $J'(u_n) - \lambda_{n} W'(u_n) \rightarrow 0.$
\end{remark}
\begin{definition}
For $\lambda \in \mathbb{R}^{+}$, we define $A_\lambda : X \rightarrow X'$ as
\[A_\lambda = J' + \lambda W'_{2}.\]
\end{definition}
\noi The following lemma is motivated by Szulkin and Willem \cite[Lemma 4.3]{Szulkin1998}.
\begin{lemma} \label{convergence lemma}
If $u_{n} \rightharpoonup u  ~in ~X ~and~\langle A_{\lambda}(u_{n}), u_{n}-u \rangle \rightarrow 0$, then $ u_{n} \rightarrow u$ in X.
\end{lemma}
\begin{proof}
Clearly, $\langle A_{\lambda}(u_{n})- A_{\lambda}(u), u_{n}-u \rangle \rightarrow 0.$ 
{We can write $\langle A_{\lambda}(u_{n})- A_{\lambda}(u), u_{n}-u \rangle = B_n + \lambda C_n, $ where $B_n = \langle J'(u_n) - J'(u), u_n -u \rangle $ and $C_n = \langle W'_{2}(u_n) - W'_{2}(u), u_n -u \rangle$.
Now by using the H\"{o}lder's inequality, we have}
\begin{align*}
 {\frac{C_n}{p}} &=  \int_{\mathbb{R}^{N}} w_{2} (|u_{n}|^{p-2}u_{n} - |u|^{p-2}u)(u_{n}-u)\, \dx \\
 &= \int_{\mathbb{R}^{N}} w_{2} (|u_{n}|^{p}+ |u|^{p} -|u_{n}|^{p-2}u_{n}u - |u|^{p-2}u u_{n}) \dx \\
 &=\int_{\mathbb{R}^{N}} w_{2} (|u_{n}|^{p}+ |u|^{p})\dx - \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p-2}u_{n}u \,\dx - \int_{\mathbb{R}^{N}} w_{2}|u|^{p-2}u u_{n}\, \dx\\
 &\geq \int_{\mathbb{R}^{N}} w_{2} (|u_{n}|^{p}+ |u|^{p})\dx - \left( \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p} \,\dx \right)^{\frac{p-1}{p}} \left( \int_{\mathbb{R}^{N}} w_{2}|u|^{p} ~\dx \right)^{\frac{1}{p}}\\
 &\qquad -\left( \int_{\mathbb{R}^{N}} w_{2}|u|^{p} ~\dx \right)^{\frac{p-1}{p}} \left( \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p} ~\dx \right)^{\frac{1}{p}}\\
 &= \left[ \left( \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p} ~\dx \right)^{\frac{p-1}{p}} - \left( \int_{\mathbb{R}^{N}} w_{2}|u|^{p} ~\dx \right)^{\frac{p-1}{p}} \right] \left[ \left( \int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p} ~\dx \right)^{\frac{1}{p}} - \left( \int_{\mathbb{R}^{N}} w_{2}|u|^{p} ~\dx \right)^{\frac{1}{p}} \right] \geq 0.
 \end{align*}
 %\tr{"we can try to Remove the cross used for multiplication"}
Now
\begin{align*}
     \frac{B_n}{p} =&\int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \left( \frac{|u_{n}(x)-u_{n}(y)|^{p-2}(u_{n}(x)-u_{n}(y))}{|x-y|^{N+sp}} - \frac{|u(x)-u(y)|^{p-2}(u(x)-u(y))}{|x-y|^{N+sp}}  \right) \\
    &\hspace{3cm} \left(u_{n}(x)-u(x)-u_{n}(y)+u(y)\right) \,\dxy \\
    &= \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy + \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy\\
    & \hspace{1cm}- \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}}  \frac{|u_{n}(x)-u_{n}(y)|^{p-2}(u_{n}(x)-u_{n}(y))(u(x)-u(y))}{|x-y|^{N+sp}}\dxy \\
    & \hspace{2cm} - \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x)-u(y)|^{p-2}(u(x)-u(y)) (u_{n}(x)-u_{n}(y))}{|x-y|^{N+sp}} \dxy\\
    % &\int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \bigg( \frac{|u_{n}(x)-u_{n}(y)|^{p-2}(u_{n}(x)-u_{n}(y))}{|x-y|^{N+sp}} - \frac{|u(x)-u(y)|^{p-2}(u(x)-u(y))}{|x-y|^{N+sp}}  \bigg) \\
    % &~~~~~~~~~~~~~~~~~~~.\big(u_{n}(x)-u(x)-u_{n}(y)+u(y)\big) ~\dxy \\
\end{align*}
\begin{align*}
    &\geq \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy + \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy \\
    &\hspace{1cm} - \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{p-1}{p}}  \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{1}{p}} \\
    &\hspace{1.5cm} - \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{p-1}{p}}  \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{1}{p}}\\
    &= \bigg[ \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{p-1}{p}}   - \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{p-1}{p}}       \bigg] \\
    &\hspace{1cm}\bigg[ \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{1}{p}}   - \bigg( \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy \bigg)^{\frac{1}{p}}       \bigg] \geq 0. 
\end{align*}
%\tr{"Remove the dots used for multiplication"}
{ Since $\langle A_{\lambda}(u_{n})- A_{\lambda}(u), u_{n}-u \rangle \longrightarrow 0$ as $n \rightarrow \infty$ and the sequences $B_n$ and $C_n$ are non-negative, we get
\[ B_n \rightarrow 0 \text{ and }  C_n \rightarrow 0 \text{ as } n \rightarrow \infty. \] }
% $$\int_{\mathbb{R}^{N}} w_{2} (|u_{n}|^{p-2}u_{n} - |u|^{p-2}u)(u_{n}-u) \dx ~ \rightarrow 0~ ~\text{as}~n \rightarrow \infty. $$
This further implies
\[\int_{\mathbb{R}^{N}} w_{2}|u_{n}|^{p} ~\dx \rightarrow \int_{\mathbb{R}^{N}} w_{2}|u|^{p} ~\dx,  \]
and
\[ \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x) - u_{n}(y)|^{p}}{|x-y|^{N+sp}} \dxy \rightarrow \int_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x) - u(y)|^{p}}{|x-y|^{N+sp}} \dxy. \]
Hence $\|u_{n}\|_{X} \rightarrow \|u\|_{X}$ and therefore $u_{n} \rightarrow u $ in X.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
{{\bf Notes:} \color{blue} Source Bonder's article page no.16  
$$\xi_{n} = \frac{|u_{n}(x)-u_{n}(y)|^{p-2} (u_{n}(x)-u_{n}(y))}{|x-y|^{\frac{N+sp}{p'}}} \in L^{p'}(\mathbb{R}^{N} \times \mathbb{R}^{N})$$  
where $p' = \frac{p}{p-1}$ and $\{ \xi_{n} \}$ is bounded in $L^{p'}(\mathbb{R}^{N} \times \mathbb{R}^{N})$. Also $ \frac{u(x)-u(y)}{|x-y|^{\frac{N}{p} + s}} \in  L^{p}(\mathbb{R}^{N} \times \mathbb{R}^{N})$.\\
Therefore, by Holder's inequality, we have 
$$\iint_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x)-u_{n}(y)|^{p-2} (u_{n}(x)-u_{n}(y))}{|x-y|^{\frac{N+sp}{p'}}}. \frac{(u(x)-u(y))}{|x-y|^{\frac{N}{p} + s}} dxdy$$
$$ \leq  \bigg( \iint_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u_{n}(x)-u_{n}(y)|^{p}}{|x-y|^{N+sp}}dxdy \bigg)^{\frac{p-1}{p}}. \bigg( \iint_{\mathbb{R}^{N} \times \mathbb{R}^{N}} \frac{|u(x)-u(y)|^{p}}{|x-y|^{N+sp}}dxdy \bigg)^{\frac{1}{p}} $$
Hence, H\"{o}lder's inequality in the above proof is verified. }
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
For $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$, the map $W'_{1} : X \rightarrow X' $ is compact.
\end{lemma}

\begin{proof}
Let $u_{n} \rightharpoonup u$ in $X$ and $v \in X$. For $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$, by Theorem \ref{H1} we have 
\begin{equation} \label{Sobolev type inequality}
    \| w_{1}^{\frac{1}{p}} u \|_{p}  \leq C \|w_{1}\|^{\frac{1}{p}}_{\mathcal{H}_{s,p}(\R^N)} \|u\|_{s,p},
\end{equation}  
where the constant $C>0$ depends on $N,s,p$ only and independent of $u$. Thus, we use H\"{o}lder's inequality to obtain
\begin{align*}
    |\langle W_{1}'(u_n) - W'_{1}(u), v \rangle|
    &\leq ~\int_{\mathbb{R}^{N}} w_{1} |( |u_{n}|^{p-2}u_{n} - |u|^{p-2}u)| |v| \dx  \\
    &\leq  \bigg(\int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx \bigg)^{\frac{p-1}{p}}  \bigg(\int_{\mathbb{R}^{N}} w_{1} |v|^{p} \dx \bigg)^{\frac{1}{p}} \\
    &\leq C~ \|w_{1}\|^{\frac{1}{p}}_{\mathcal{H}_{s,p}(\R^N)} \|v\|_{s,p} \bigg(\int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx \bigg)^{\frac{p-1}{p}}.
\end{align*}
Thus
$$ \|W'_{1}(u_{n}) - W'_{1}(u)\| \leq C ~\|w_{1}\|^{\frac{1}{p}}_{\mathcal{H}_{s,p}(\R^N)} \bigg(\int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx \bigg)^{\frac{p-1}{p}}.$$
%\tr{"Remove the dots used for multiplication"}
Now, it is sufficient to show that
$$\bigg(\int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx \bigg)^{\frac{p-1}{p}} \longrightarrow 0 ~ as~n \rightarrow \infty.$$
Let $\epsilon>0$ and $w_{\epsilon} \in C_{c}^{\infty}(\mathbb{R}^{N})$ be arbitrary.
\begin{equation} \label{Integral with w}
     \int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx \hspace{86mm}
\end{equation} 
$$
   = \int_{\mathbb{R}^{N}} w_{\epsilon} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx + \int_{\mathbb{R}^{N}} (w_{1} -w_{\epsilon}) |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx.
$$
First, we estimate the second Integral. Since $\{u_{n}\}$ is bounded in $X$, 
$$ K := \sup_{n} (\|u_{n}\|_{s,p}^{p} + \|u\|_{s,p}^{p}) < \infty. $$
Now
\begin{align*}
    \int_{\mathbb{R}^{N}} (w_{1} -w_{\epsilon}) |(|u_{n}|^{p-2}u_{n} &-|u|^{p-2}u)|^{\frac{p}{p-1}} \dx\\
    &\leq \int_{\mathbb{R}^{N}} (w_{1} -w_{\epsilon}) \left(|u_{n}|^{p-1} +|u|^{p-1}\right)^{\frac{p}{p-1}} \dx \\
    &\leq 2^{\frac{1}{p-1}} \left( \int_{\mathbb{R}^{N}} (w_{1} -w_{\epsilon}) |u_{n}|^{p} \dx + \int_{\mathbb{R}^{N}} (w_{1} -w_{\epsilon})|u|^{p} \dx \right) \\
    &\leq 2^{\frac{1}{p-1}} C  \|w_{1} - w_{\epsilon}\|_{\mathcal{H}_{s,p}(\R^N)} \left(\|u_{n}\|_{s,p}^{p}+ \|u\|_{s,p}^{p}\right)\\
    &\leq 2^{\frac{1}{p-1}} C K \|w_{1} - w_{\epsilon}\|_{\mathcal{H}_{s,p}(\R^N)}.
\end{align*}
%\tr{"Remove the dots used for multiplication"}
Now since $w_{1} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N})$, from the definition of $\mathcal{H}_{s,p,0}(\mathbb{R}^{N})$, we can choose $w_{\epsilon} \in C_{c}^{\infty}(\mathbb{R}^{N})$ such that
$$ 2^{\frac{1}{p-1}} K \|w_{1} - w_{\epsilon}\|_{\mathcal{H}_{s,p}(\R^N)} < \frac{\epsilon}{2C}. $$
Hence, we can choose $w_\epsilon$ suitably such that the second Integral in (\ref{Integral with w}) can be made less than $\frac{\epsilon}{2}$. The space X is compactly embedded into $L^{p}_{loc}(\mathbb{R}^{N})$, therefore the first integral converges to $0$ up to a subsequence $\{u_{n_{k}}\}$ of $\{u_{n}\}$. Thus we obtain $k_{0} \in \mathbb{N}$ such that,
$$  \int_{\mathbb{R}^{N}} w_{1} |(|u_{n_{k}}|^{p-2}u_{n_{k}} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx < \epsilon, ~~~\forall ~k>k_{0}. $$
We conclude by the uniqueness of the limit of subsequence that
$$  \int_{\mathbb{R}^{N}} w_{1} |(|u_{n}|^{p-2}u_{n} -|u|^{p-2}u)|^{\frac{p}{p-1}} \dx ~\longrightarrow ~0 ~~as~~n \rightarrow \infty.  $$
Hence, the proof.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% \begin{lemma}
% The map $W'_{1} : X \rightarrow X' $ is compact.
% \end{lemma}
% \begin{proof}
% Let $u_{n} \rightharpoonup u$ in X and $v \in X$. Then
% $$ (|u_{n}|^{p-2}u_{n} - |u|^{p-2}u) \in L^{\frac{p_{s}^{*}}{p-1}, \frac{p}{p-1}}(\mathbb{R}^{N}).$$

% \begin{equation} \label{Sobolev type inequality}
%     \| w_{1}^{\frac{1}{p}} u \|_{p}  \leq C \|w_{1}\|^{\frac{1}{p}}_{\mathcal{H}_{s,p}(\R^N)} [u]_{s,p}
% \end{equation}  
% \begin{align*}
%     <W_{1}'(u_n) - W'_{1}(u), v>~~ = ~\int_{\mathbb{R}^{N}} w_{1} ( |u_{n}|^{p-2}u_{n} - |u|^{p-2}u) v dx \hspace{17mm} \\
%     = ~\int_{\mathbb{R}^{N}} w_{1} |u_{n}|^{p-2}u_{n}v dx - \int_{\mathbb{R}^{N}} w_{1}|u|^{p-2}u v dx.
% \end{align*}
% By standard integration theory, we get
% $$\int_{\mathbb{R}^{N}} w_{1} |u_{n}|^{p-2}u_{n}v dx \rightarrow \int_{\mathbb{R}^{N}} w_{1} |u|^{p-2}uv dx ~~({\color{red} ??})$$
% Since $0\leq w_{1} \in L^{1}_{loc}(\mathbb{R}^{N}) $ and $ D^{s,p}(\mathbb{R}^{N}) \subset \subset L^{p}(w_{1};dx)$. {\color{red} (See page no.16 first convergence in Bonder's article ).}
% Hence, the result follows immediately.\\
% \end{proof}
% \fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Further, we prove that the (PS) condition is satisfied by the functional $J$ on $\mathbb{S}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}
The functional $J$ satisfies the Palais-Smale (PS) condition on $\mathbb{S}$.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{proof}
We consider a sequence $\{ u_n \}$ in $\mathbb{S}$ such that $J(u_n) \rightarrow \lambda$ and $J'(u_n) \rightarrow 0.$ Thus by Remark \ref{rem2} , there exists a sequence $\{  \lambda_{n} \}$ such that
\begin{equation} \label{Palais smale condition}
   J'(u_n) - \lambda_{n} W'(u_n) \rightarrow 0 \text{ in }X' \text{ as } n \rightarrow \infty. 
\end{equation}
Since $J(u_n)$ is bounded, using the inequalities $\int_{\mathbb{R}^{N}} w |u_{n}|^{p} dx > 0$, and 
\begin{align} \label{L1}
 \int_{\mathbb{R}^{N}} w_{2} |u_{n}|^{p} \dx  &<  \int_{\mathbb{R}^{N}} w_{1} |u_{n}|^{p} \dx  \leq C \|w_{1}\|_{\mathcal{H}_{s,p}(\R^N)} \|u_{n}\|_{s,p}^{p},
\end{align}
we derive that the sequence $\{W_{2}({u_n}) \}$ is bounded in $\R$. So the sequence $\{ u_{n} \}$ is bounded in X, and since $X$ is reflexive, the sequence $\{ u_{n} \}$ admits a weakly convergent subsequence, i.e., there exists a $u \in X$ such that $u_n \rightharpoonup u$ {in X} up to a subsequence. {Since $X$ is continuously embedded in $\D^{s,p}(\R^N)$, the map $W_1$ is also compact on X. Thus, we obtain $W_1(u_n) \rightarrow W_1(u)$ in $\R$}. Now Fatou's Lemma yields
\begin{align} \label{L2}
    \int_{\mathbb{R}^{N}} w_{2} |u|^{p} \dx \leq  \liminf_{n} \int_{\mathbb{R}^{N}} w_{1} |u_n|^{p} \dx - 1 = \int_{\mathbb{R}^{N}} w_{1} |u|^{p} \dx - 1.
\end{align}
Thus $\int_{\mathbb{R}^{N}} w |u|^{p} \dx \geq 1 $ and hence $ u \neq 0.$ Further, $\lambda_{n} \rightarrow \lambda$ as $n \rightarrow \infty$, since $$ p (J(u_n) - \lambda_n)  = \langle J'(u_n) - \lambda_n W'(u_n), u_n \rangle ~ \ra ~0, \text{ as } n \ra \infty.$$  %( as~\langle W'(u_{n}),u_{n} \rangle = p)}$$
Now we write (\ref{Palais smale condition}) as $$ A_{\lambda_n}(u_n) - \lambda_n W'_{1}(u_n) \rightarrow 0 ~ as~n \rightarrow \infty.$$
Since $\lambda_n \rightarrow \lambda$, we obtain {$A_{\lambda_n}(u_n) - A_{\lambda}(u_n) \rightarrow 0$ in $X'$.} Further the compactness of $W'_{1}$ implies the strong convergence of $A_{\lambda}(u_n)$ and hence $\langle A_{\lambda}(u_n), u_{n} - u \rangle \rightarrow 0$. Since {$u_{n} \rightharpoonup u$ in $X$,} using Lemma \ref{convergence lemma} one obtains $u_{n} \rightarrow u$ in X.
 \end{proof} 
Next, we state the following Lemma:
%\begin{lemma}[\cite[Lemma 5.9]{anoop-p}]
\begin{lem}[{{\cite[Lemma 5.9]{{anoop-p}}}}]% \label{Bonder lemma two}
The set $\Gamma_{n}$ is non-empty for each $n \in \mathbb{N}$.
\end{lem}

Finally, we prove the existence of an infinite set of eigenvalues for (\ref{Weighetd eigenvalue problem}) by employing the Ljusternik-Schnirelmann theorem on $C^1$-manifold.
\begin{proof}[Proof of theorem \ref{Infinite eigenvalue}]
We know that the functional $J$ and the set $\mathbb{S}$ satisfy all the conditions of Theorem \ref{Ljusternik}. Therefore, we get $\gamma(K_{\lambda_{j}}) \geq 1$ for each $j \in \mathbb{N}$. Thus $K_{\lambda_{j}} \neq \emptyset$ and hence there exists $u_{j} \in \mathbb{S}$ such that $J'(u_{j}) = 0$ and $J(u_{j}) = \lambda_{j}$. Therefore, $\lambda_{j}$ is an eigenvalue and $u_{j}$ is the corresponding eigenfunction for (\ref{Weighetd eigenvalue problem}).
Recall that X is separable \cite[Lemma 2.1]{Cui} and hence X admits a bi-orthogonal system $\{ e_{m}, e_{m}^{*}\}$ such that 
$$\overline{ \{ e_{m} : m \in \mathbb{N}  \}} = X,~ e_{m}^{*} \in X',~~\langle {e_{n}},e_{m}^{*}\rangle = \delta_{n,m}$$
$$ \langle e_{m}^{*}, x \rangle = 0,~ \forall m \implies x=0.$$
Let $E_{n} = span \{ e_{1}, e_{2}, ... ,e_{n} \}$ and let $E_{n}^{\perp} = \overline{span \{ e_{n+1}, e_{n+2}, ...  \}}$. Since  $E_{n-1}^{\perp}$ is of co-dimension $(n-1)$, for any $A \in \Gamma_{n}$ we have $A \cap E_{n-1}^{\perp} \neq \emptyset.$ Let 
$$ \mu_{n} = \inf_{A \in \Gamma_{n}} \sup_{A \cap E_{n-1}^{\perp}} J(u),~~n=1,2,...$$
Now we show that $\{ \mu_{n} \} \rightarrow \infty$. On contrary suppose that $\{ \mu_{n} \}$ is bounded, then there exists $u_{n} \in E_{n-1}^{\perp} \cap \mathbb{S}$ such that $\mu_{n} \leq J(u_{n}) <c$, for some constant $c >0$. Since $u_{n} \in \mathbb{S}$, the sequence $\{u_{n}\}$ is bounded in $X$ by using estimate (\ref{L1}). Thus $u_{n} \rightharpoonup u$ for some $u \in X$. Now by the choice of biorthogonal system, for each $m$, $\langle e_{m}^{*}, u_{n} \rangle \longrightarrow 0 ~as~ n \rightarrow \infty.$ Thus $u_{n} \rightharpoonup 0$ in X and hence $u = 0$, a contradiction to $ \int_{\mathbb{R}^{N}} w|u|^{p} \dx \geq 1$ (See the conclusion of \eqref{L2}). Therefore, $\mu_{n} \rightarrow \infty$ as $n \ra \infty$ and $\lambda_{n} \rightarrow \infty \ \text{as } n \ra \infty, \ \text{since }\mu_{n} \leq \lambda_{n}$. Moreover, the first eigenvalue is simple by Lemma \ref{Simple} and positive by Lemma \ref{Positive}. Hence, the proof is complete.
\end{proof} 
\begin{remark}
For $w_{2} \in \mathcal{H}_{s,p,0}(\mathbb{R}^{N}) \backslash \{0 \}$, a sequence of negative eigenvalues, namely, $\{\mu_{n}\}_{n \in \mathbb{N}}$ of (\ref{Weighetd eigenvalue problem}) tending to $-\infty$ exists. In addition, the first eigenvalue $ \mu_{1}$ is a simple and negative principal.
\end{remark}
